Picsou: Enabling Replicated State Machines to Communicate Efficiently

Replicated state machines (RSMs) cannot communicate effectively today as there is no formal framework or efficient protocol to do so. To address this issue, we introduce a new primitive, Cross-Cluster Consistent Broadcast (C3B) and present PICSOU, a practical implementation of the C3B primitive. PICSOU draws inspiration from networking and TCP to allow two RSMs to communicate with constant metadata overhead in the failure-free case and a minimal number of message resends in the case of failures. PICSOU is flexible and allows both crash fault tolerant and Byzantine fault tolerant consensus protocols to communicate. At the heart of PICSOU's good performance and generality is the concept of QUACKs (quorum acknowledgments). QUACKs allow nodes in each RSM to precisely determine when messages have definitely been received, or likely lost. Our results are promising: we obtain up to 24x better performance than prior solutions on microbenchmarks and applications, ranging from disaster recovery to data reconciliation.

==> algo.tex <==
\section{\Shadow{}}
\label{s:algo}
\Scrooge{} aims to efficiently implement the \CCC{} primitive without relying 
on any trusted third-party code or infrastructure and without broadcasting 
multiple copies of a message across the network.
%Prior works attempt to implement the \CCC{} primitive in following ways:
%(1) deploying trusted hardware and infrastructure,
%(2) employing zero knowledge proofs, and
%(3) concurrently sending multiple copies of each message.
%The key challenge with the use of trusted hardware is that they 
%are expected to remain honest, which makes them a sink for all attacks.
%Solutions based on zero knowledge proofs 
%are not only computationally expensive to generate, but also  and have high latencies.
%
%Alternatively, each \RSM{} can create and send multiple copies of each message, 
%but this design requires deciding which replica(s) in the \RSM{} will send the message to 
%which replica(s) in the receiver \RSM{}.
%Some \RSM{}-to-\RSM{} communication protocols opt for the hands-off {\em all-to-all} communication 
%where every replica in the sending \RSM{} sends a copy of the message to every replica in the receiving \RSM{}.
%Other protocols attempt to communicate only linear number of messages, but they 
%fall back to the all-to-all communication for recovery from Byzantine attacks.
%Moreover, these solutions expect a synchronous network.
\Scrooge{} offers the following appealing properties:
\begin{enumerate}[wide,nosep,label=(P\arabic*),ref={P\arabic*}]
\item \label{g:hetero} {\bf Heterogeneity.}
\Scrooge{} facilitates communication between two \RSM{s} with arbitrary sizes and failure models.

\item \label{g:async} {\bf Asynchrony.}
\Scrooge{} does not require a synchronous network to reliably deliver messages across \RSM{s}.

\item \label{g:single} {\bf Singularity.}
\Scrooge{} saves available bandwidth by creating zero copies of each message in the good case.

\item \label{g:recovery} {\bf Optimal Recovery.}
\Scrooge{} introduces constant-sized cumulative \quack{s} to detect and recover from failures.

\item \label{g:bidrect} {\bf Duality.}
\Scrooge{} allows both \RSM{s} to simultaneously send and receive messages;
\Scrooge{} harnesses this bi-directional pattern to piggyback acknowledgments.

\item \label{g:indepen} {\bf Independence.}
\Scrooge{} prevent an honest sender/receiver to be forever stuck with a Byzantine 
sender/receiver.

\end{enumerate}

\begin{figure}[t]
    %\vspace{-6mm}
    \centering
    \includegraphics[width=0.85\columnwidth]{end-flow.pdf}
    %\vspace{-2mm}
    \caption{An illustration of \CCC{} primitive between two \RSM{s}, which employ some consensus protocol to manage their states and
    adopt \Scrooge{} for exchanging messages.}
    \label{fig:end-flow}
\end{figure}

In Figure~\ref{fig:end-flow}, we illustrate how \Scrooge{} implements \CCC{} primitive between two \RSM{s} 
and guarantees an end-to-end data flow that meets our aforementioned properties.
For the sake of understanding, in this section, we assume that all the replicas have equal shares.
Each \RSM{} receives requests from clients and runs its choice of consensus protocol to commit those requests. 
To do so, each replica runs an instance (App) of the consensus protocol.
Post this, each replica communicates the committed requests to the co-located \Scrooge{} instance, which 
follows the \Scrooge{} protocol to send the message to a replica in the other \RSM{}.
Once the sending \Scrooge{} instance receives a cumulative \quack{} for the sent message, 
it acknowledges the receipt of the message to the co-located consensus instance.
Similarly, when the receiver receives a valid message, it forwards that message to its corresponding consensus instance.

Internally, a sender \Scrooge{} instance does the following tasks:
(1) Randomly select a receiver.
(2) Determine message to send.
(3) Send the message.
(4) Piggyback cumulative acknowledgments for received messages.
(5) Collect \quack{s} for sent messages.
%
Similarly, a receiver \Scrooge{} instance does the following tasks:
(1) Validate the received message, if invalid, discard.
(2) Send cumulative acknowledgment to the sender.
(3) Broadcast the received message in its \RSM{}.
%
Notice that \Scrooge{} is oblivious to clients and disinterested in the content of the message.


{\bf Message Format.}
To meet the desired goals, every \Scrooge{} instance expects that the 
corresponding consensus instance only forwards {\em committed} requests;
a committed request is expected to accompany a {\em proof}, which illustrates that a quorum of 
replicas in this \RSM{} have ordered this request.
However, consensus instances running on Byzantine replicas may not fulfill this requirement, 
and in \S~\ref{s:fail} we present steps to overcome various failures.
We expect the following from each honest consensus instance:
(1) It forwards all the requests that need to be sent to the other \RSM{} to its co-located Scrooge instance. 
(2) It ensures that each forwarded request is of the form $\SignMessage{m, \Seqn}{\Qusign{i}}$, 
where $m$ is a request committed at sequence number $\Seqn$ by a quorum of replicas in \RSM{} $\SMR{i}$ 
and $\Qusign{i}$ includes the digital signatures of this quorum.


{\bf Destination and Message Discovery.}
Although each \Scrooge{} instance has access to all the committed requests, 
to meet the promise of zero copy transmission,
we ask each instance to send a {\em unique} committed request to the other \RSM{}.
This uniqueness also brings forth three key challenges:
(1) which request to send, 
(2) whom to send, and
(3) how to detect successful transmission.

We handle the first challenge by evenly dividing all the messages to be sent across all the 
\Scrooge{} instances.
To do so, we perform the $\bmod$ operation as follows: 
$\Seqn \bmod j$, where the message with sequence number $\Seqn$ is sent by $j$-th \Scrooge{} instance.
%
To meet the next two challenges, we need to determine the destination for each message. 
A naive way to do so would be to enable {\em static pairing} where each sender is paired 
with one receiver (replica at the other \RSM{}) and the sender sends all its messages to this one receiver.
There is a key limitation of static pairing: 
either the sender or the receiver may act Byzantine, which makes it impossible to determine if a message 
has been received at the destination \RSM{}.

As a result, our \Scrooge{} protocol dynamically switches pair using the round-robin protocol.
A $j$-th \Scrooge{} instance determines the identity of the next receiver by running the mod operation 
over the identifier of the previous receiver:
\begin{equation}
 \text{next receiver} =  (j + 1) \bmod \n{i}
\end{equation}
where $j$ is the identifier of the previous receiver and $\n{i}$ are the number of replicas in the receiving \RSM{}.
To ensure every instance starts with a different receiver, the first receiver for the $j$-th 
instance is the replica with identifier $j$.

Next, we illustrate the three step \Scrooge{} protocol.
For simplicity, we will assume that replicas in \RSM{} $\SMR{1}$ (sender \RSM{}) 
want to communicate messages to replicas in \RSM{} $\SMR{2}$ (receiver \RSM{});
this protocol can be used to send messages in either directions.
Further, we assume that all the committed requests received by \Scrooge{} instances 
have continuous sequence numbers;
in \S~\ref{ss:cum-quack}, we show how to trivially eliminate this requirement.


\subsection{Message Transmission}
\label{ss:transmit}
When the $j$-th replica $\Replica{1}{j}$ of \RSM{} $\SMR{1}$ receives a committed request
$\SignMessage{m}{\Qusign{1}}$ from the co-located consensus instance, 
it determines if it is responsible for sending this message. 
To do this, $\Replica{1}{j}$ takes the sequence number of this request (say $\Seqn$) 
and runs the $\bmod$ operation.
If this is the case, $\Replica{1}{j}$ determines the receiver for this message using 
the destination discovery procedure described earlier. 
Assume replica $\Replica{2}{l}$ of the \RSM{} $\SMR{2}$ is the intended receiver.
Finally, $\Replica{1}{j}$ creates a message $\SignMessage{m, \Seqn}{\Qusign{1}}$ and 
sends this message to $\Replica{2}{l}$.

Note: 
(1) $\Replica{1}{j}$ uses \Name{Mac} to sign the message $\SignMessage{m, \Seqn}{\Qusign{1}}$ 
prior to sending it to $\Replica{2}{l}$; this $\Name{Mac}$ prevents an adversary from 
intercepting the message and modifying its content.
(2) Each message is sent by only one replica of \RSM{} $\SMR{1}$, thereby, 
zero copy transmission.


\subsection{Message Reception}
When the $l$-th replica $\Replica{2}{l}$ receives a message $\SignMessage{m, \Seqn}{\Qusign{1}}$ 
from a replica in \RSM{} $\SMR{1}$, it checks if $\Qusign{1}$ includes signatures of a 
quorum of replicas of \RSM{} $\SMR{1}$ for message $m$. 
If this is the case, $\Replica{2}{l}$ assumes that $m$ is a valid request committed 
at sequence number $\Seqn$ and sends an acknowledgment to replica $\Replica{1}{l}$.
Finally, replica $\Replica{2}{l}$ {\em broadcasts} this message $\SignMessage{m, \Seqn}{\Qusign{1}}$ in its \RSM{};
broadcast helps other replicas in the \RSM{} to receive the message and acknowledge 
its receipt in the future.

Note: 
if the receiver $\Replica{2}{l}$ also has some message (any committed request that it 
received from its \RSM $\SMR{2}$) 
to send to replica $\Replica{1}{j}$,
it can simply piggyback the acknowledgment message with this message.


\subsection{Cumulative Quorum Acknowledgment}
\label{ss:cum-quack}
The key ingredient behind \Scrooge's aforementioned six appealing properties is its 
cumulative quorum acknowledgments (\quack{}).
Cumulative \quack{s} are constant-sized and help all the sending \RSM{}
replicas determine 
whether at least one honest party at the receiving \RSM{} received the message.
\Scrooge{} provides all the sending \RSM{} replicas (not only the sender)  
acknowledgments for each message sent so that they can detect any failures.

Without cumulative \quack{s}, for each message sent, each sending \RSM{} replica 
would require acknowledgments from a quorum of replicas of the receiving \RSM{}.
As up to $\f{2}$ replicas of the receiving \RSM{} can act Byzantine, the quorum size  
is $\f{2}+1$, which proves that at least one honest party received the message.
Clearly, sending $\f{2}+1$ acknowledgments per message will exhaust the available bandwidth.

\Scrooge{} aggregates multiple acknowledgments together and 
sends a single cumulative acknowledgement.
Specifically, each receiver maintains a contiguous set of messages $\SAck{}$.
Prior to receiving any message, each receiver initializes its set $\SAck{}$ with a {\em null} element ($\phi$).
Whenever a replica receives a message $m$ with sequence number $\Seqn$ from the sending \RSM{}, 
it adds it to the set $\SAck{}$
if $\Seqn$ is one more than the largest sequence number in $\SAck{}$; the first addition to $\SAck{}$ is message 
with $\Seqn = 0$.
Otherwise, it holds adding the message with higher sequence number until the messages with lower
sequence number arrives.

Post this, the receiver finds the last sequence number (also the highest) in the set $\SAck{}$ (say $\Seqn$)
and sends a message $\Ack{\Seqn}$ to the sender.
Notice that initially, receivers send message $\Ack{\phi}$ until they have access to a message with sequence number $\Seqn=0$.
Once it receives the message with $\Seqn=0$, for any messages it receives in the future, 
it sends an acknowledgment $\Ack{p}$, if $\SAck{}$ includes all the messages between $\Seqn=0$ and $\Seqn=p$.
%
%For example, assume replica $\Replica{2}{l}$ has already acknowledged message $\SignMessage{m,5}{\Qusign{1}}$
%and is yet to acknowledge messages $\SignMessage{m,6}{\Qusign{1}}$ and $\SignMessage{m,7}{\Qusign{1}}$ 
%when it receives message $\SignMessage{m,8}{\Qusign{1}}$ from replica $\Replica{1}{j}$.
%Hence, it creates a cumulative acknowledgment $\Ack{8}$ and sends it to $\Replica{1}{j}$.
%
Thus, when the sender receives a cumulative acknowledgment (say $\Ack{p}$), it determines
that messages up to sequence number $p$ have been received by at least one replica in the receiving \RSM{}.
When does this sender marks the message with sequence number $\Seqn$ 
received by at least one honest replica in the receiving \RSM{}? 
When it receives cumulative acknowledgements for messages with sequence number $\ge p$
from at least $\f{2}+1$ distinct receivers.
This set of $\f{2}+1$ acknowledgments for a message $m$ is what we term as a \quack{} for $m$.

%Note: although each replica sends each message to only one receiver, 
%it is able to create a \quack{} as it runs our round robin algorithm to determine the destination for each message.
%Consequently, each replica ends up sending some message to each replica in the other \RSM{}.



\section{Weighted \RSM{s} -- Stakes}
\label{s:stake}
Until now, we assumed that all the replicas have equal shares or stakes. 
However, several existing systems allow replicas to have different shares, 
where a replicas' share determines its decision making power in the \RSM{}.
This brings forth several new challenges for our \Scrooge{} protocol.
\begin{enumerate}
    \item For each \RSM{}, the notations $\n{}$ and $\f{}$ refer to the total 
    stake and Byzantine stake and not the traditional terminology for referring to 
    number of replicas.
    This implies that the total $\n{}$ stake is distributed among less than $\n{}$ replicas.

    \item Each sender with stake $> 1$ would have to send multiple consecutive messages 
    to one receiver.
    As a result, the acknowledgments from the receiving \RSM{} will also be proportional 
    to the stake of the receiver.

\end{enumerate}

To allow our \Scrooge{} protocol to handle such weighted \RSM{}, we need to modify 
the way a sender discovers messages to send, intended receiver, and counting cumulative \quack{}.

\begin{figure}[t]
    \begin{myprotocol}
	\INITIAL{Initialization:}{\newline
	{%\color{orange}
	// $\SMR{1} :=$ \RSM{} of the replica calling this function.\newline
	// $\SMR{j} :=$ Receiver \RSM{}.
	}}
	\vspace{1mm}

	\FUNC{sws}{message identifier: $\Seqn$; sorted List: $\SList$}
		\STATE $\DList$ $:=$ $\SList$ (Temporary list).
            \STATE $\n{j}$ $:=$ Total stake of $\SMR{j}$.
            \STATE $orig$ $:=$ $\Seqn \bmod \n{j}$
            \STATE $iter$ $:=$ $\lfloor \Seqn / \n{j} \rfloor$
            \STATE $dest$ $:=$ $(orig + iter) \bmod \n{j}$.
		\STATE {\bf return} $dest$.
	\ENDFUNC
	\SPACE
    \end{myprotocol}
    \caption{Sharewise Scheduler to identify the message receivers.}
    \label{func:sws}
\end{figure}



{\bf Dynamic Sharewise Scheduler.}
First, we modify the protocol for selecting the destination for a message. 
We can no longer use the round robin protocol $+$ $\bmod$ operation (\S~\ref{s:algo}) 
as it is oblivious to the total shares of each \RSM{} and the shares of each replica and 
sends all the replicas in the receiving \RSM{} an equal number of messages.
This in turn would send more messages to Byzantine receivers, which can deteriorate the 
performance of the \Scrooge{} protocol.

To this end, we design a Dynamic Sharewise Scheduler (\SWS), which builds on top of the 
Completely Fair Scheduler (\CFS{})~\cite{cfs} algorithm.
Prior to running the \SWS{} scheduler, we normalize the total shares of each \RSM{}. 
with their {\em least common multiple} (LCM). 
For example, assume $\n{1}$ and $\n{2}$ are the total shares of \RSM{} $\SMR{1}$ and $\SMR{2}$, 
and $\n{1}\times\n{2}$ is the LCM, then normalizing the shares requires multiplying 
the shares of each replica in $\SMR{1}$ with $\n{2}$ and the shares of each replica in $\SMR{2}$ with $\n{1}$.
%As we will see below, this normalization eases the mapping between replicas of $\SMR{1}$ and $\SMR{2}$.

Next, each sender calls the \SWS{} protocol (Figure~\ref{func:sws})
with the sequence number of the message ($\Seqn$) as input.
The \SWS{} protocols returns $dest$ as output, which states the ``share''
responsible for receiving this message.
Finally, the sender translates the $dest$ share to the identity of corresponding receiver replica, 
which is a trivial task given the knowledge of shares and identifiers of all replicas.
Instead of returning the identifier of the replica, \SWS{} returns the responsible 
share because the protocol views the total share $\n{j}$ of an \RSM{} $\SMR{j}$ as $\n{j}$ distinct identities.


\subsection{Weighted \Scrooge{}}
With weighted \RSM{s}, we need to slightly modify our basic \Scrooge{} protocol.
The {\em message transmission} step remains unchanged except that each sender calls the dynamic \SWS{} scheduler  
to identify the receiver for a message. 
As earlier, for deciding if a replica with identifier $l$ and share $\share{j}$ 
of the \RSM{} $\SMR{i}$ is responsible for sending the message with sequence number $\Seqn$, 
we perform the operation $\Seqn \bmod \n{i}$.
However, instead of providing the identifier for a replica, each sender receives the information about 
the responsible share, which is trivial to map to the sender identifier.

Similarly, {\em message reception} step remains unchanged.
However, there is a small change in the way a sender reaches a cumulative \quack{}. 
In the basic \Scrooge{} protocol, the sender waits for cumulative acknowledgment 
messages for message $m$ from $\f{2}+1$ distinct replicas of the receiving \RSM{} $\SMR{2}$ 
before concluding that $m$ has been successfully received by at least one honest 
replica of $\SMR{2}$.
This principle may not apply when the \RSM{s} are weighted because the total number of 
distinct replicas are no longer bounded by notations $\n{}$ and $\f{}$. 
Thus, each cumulative acknowledgment message is now weighted; 
acknowledgment message from a $l$-th replica with share $\share{l}$ has a weight $\share{l}$.
As a result, the sender marks a message $m$ received at \RSM{} $\SMR{j}$ when 
the total weight of cumulative \quack{} for $m$ from $\SMR{j}$ is equal to $\f{j}$.




%\item {\bf Transmit.}
%On calling the function \SWS{}, each replica $\Replica{i}{l}$ receives a list of replicas ($\DList$) it needs 
%to send messages.
%\Scrooge{} requires $\Replica{i}{l}$ to send each replica in $\DList$ a unique message from its $\Sbuf{l}$.
%To determine which messages from $\Replica{i}{l} $ each replica in $\DList$ receives, $\Replica{i}{l}$ calls the function 
%{\bf transmit} in Figure~\ref{func:sws}.
%In this function, we use the extracted messages to refer to messages with the least sequence number.
%
%\begin{example}
%Say the call to function $\SWS{}$ by replica $\Replica{i}{l}$ with share $\share{l} = 3$ returned 
%$\DList{} = \{\Replica{j}{r}, \Replica{j}{s} \}$, such that $\share{r} = 2$ and $\share{s} = 3$.
%Assume 
%\[\Sbuf{l} = \{ \SignMessage{m,k}{\Qusign{i}}, \SignMessage{m',k'}{\Qusign{i}}, \SignMessage{m^\circ,k^\circ}{\Qusign{i}}, \SignMessage{m^{\star},k^{\star}}{\Qusign{i}},... \}\]
%such that $k < k' < k^\circ < k^\star$.
%After sending every three messages from $\Sbuf{l}$, $\Replica{i}{l}$ loops back to $\DList$.
%Specifically, $\Replica{i}{l}$ extracts $\SignMessage{m,k}{\Qusign{i}}$ and $\SignMessage{m',k'}{\Qusign{i}}$ and sends to $\Replica{j}{r}$, 
%extracts $\SignMessage{m^\circ,k^\circ}{\Qusign{i}}$ and sends to $\Replica{j}{s}$, and cycles back to $\Replica{j}{r}$
%and sends it $\SignMessage{m^{\star},k^{\star}}{\Qusign{i}}$.
%As a result, in each cycle $\Replica{i}{l}$ sends $\Replica{j}{s}$ only one message even though $\share{s} = 3$.
%
%\end{example}

%\item {\bf Cumulative Acknowledgments.}
%If the two \RSM{s} are participating in bidirectional communication streams,  
%it is possible that $\Replica{i}{l}$ may have received messages from some replicas in \RSM{} $\SMR{j}$.
%We require $\Replica{i}{l}$ to acknowledge each message it received from \RSM{} $\SMR{j}$. 
%To conserve bandwidth, instead of sending an acknowledgment for each received message, 
%\Scrooge{} requires $\Replica{i}{l}$ to create cumulative acknowledgments and {\em piggyback} them with 
%the outgoing messages.
%
%Prior to sending a message,
%each replica searches its list $\SAck{l}$ for the longest contiguous set of acknowledgments.
%The last acknowledgment of this contiguous list is considered as the cumulative acknowledgment for all the 
%messages in this list. 
%Assume $\Ack{1}, \Ack{2}, ... , \Ack{k'}$ is one such longest contiguous set of acknowledgments.
%If this is the case, then $\Replica{i}{l}$ appends acknowledgment $\Ack{k'}$ to the outgoing message.

%\item {\bf \em Receipt.}
%When the $r$-th replica $\Replica{j}{r}$ of the $j$-th \RSM{} receives the 
%message $\SignMessage{m, k}{\Qusign{i}}$ and acknowledgment $\Ack{k'}$ from replica $\Replica{i}{l}$ of \RSM{} $\SMR{i}$,
%it broadcasts the message and acknowledgment to all the replicas in its \RSM{}.
%Replica $\Replica{j}{r}$ also uses the piggybacked cumulative acknowledgment $\Ack{k'}$ to determine the fate of the 
%messages sent by its \RSM{} $\SMR{j}$ to replicas of \RSM{} $\SMR{i}$.
%Specifically, replica $\Replica{j}{r}$ updates the data-structure $\RAck{r}{}$ as follows:
%for all the values $u \in [1,k']$, increment $\RAck{r}{u}$ by one.
%If any $\RAck{r}{u}$ reaches the count $\f{j}+1$, it marks the message $\SignMessage{m, u}{\Qusign{j}}$ 
%as {\em delivered}.
%We require replica $\Replica{j}{r}$ to keep track of the last delivered message  (one with highest sequence number till now)
%in a variable $\highest{}$.

%Say the sequence number for $m$ be $l$.
%If $\Replica{\Cluster{X}}{i}$ has received all the messages with sequence number less than $l$ from cluster $\Cluster{Y}$, 
%it goes ahead and processes $m$. 
%If this is not the case, then $\Replica{\Cluster{X}}{i}$ stores $m$ at the index $l$ in $\Rbuf{}$.
%This $\Rbuf{}$ helps $\Replica{\Cluster{X}}{i}$ to determine the contiguous sequence of messages it has received to send a cumulative 
%acknowledgment in future.
%
%Each message $m'$ received by $\Replica{\Cluster{X}}{i}$ also includes a cumulative acknowledgment ($\Ack{k}$). 
%This is the acknowledgment from the replica $\Replica{\Cluster{Y}}{j}$ (sender of $m'$).
%Through this $\Ack{k}$, $\Replica{\Cluster{Y}}{j}$ wants to inform that it has received all the messages till sequence number $k$ 
%from cluster $\Cluster{X}$.
%This allows $\Replica{\Cluster{X}}{i}$ to increment the {\em counter} for each message with sequence number $\le k$ 
%in its $\Sbuf{}$ and $\Hbuf{}$.
%When the counter for any message reaches $\f{\Replicas{}}+1$, the corresponding message is removed from $\Sbuf{}$ or $\Hbuf{}$.
%We call this message to be {\em majority acknowledged}.


%\begin{figure}[t]
%    \begin{myprotocol}
%	\INITIAL{Initialization:}{\newline
%	{%\color{orange}
%	// $\SMR{i} :=$ \RSM{} of the replica calling this function.\newline
%	// $\SMR{j} :=$ Receiver \RSM{}.
%	}}
%	\vspace{1mm}
%
%	\FUNC{sws}{caller's identifier: $a$}
%		\STATE $\SList :=$ Sorted list of replicas of $\SMR{j}$ on the basis of shares.
%		\FOR{$l$ : $1$ to $\n{i}$}
%			\STATE $\share{l} :=$ share of replica $\Replica{i}{l}$.
%			\WHILE{$\share{l} \ne 0$} 
%				\STATE $\Replica{j}{r} :=$ replica with the smallest share in $\SList$.
%				\STATE $\share{r} :=$ share of replica $\Replica{j}{r}$.
%				\IF{$\share{l} > \share{r}$}
%					\STATE $\share{l} := \share{l} - \share{r}$.
%					\STATE Remove $\Replica{j}{r}$ from $\SList$.
%				\ELSE
%					\STATE $\share{r} := \share{r} - \share{l}$.
%					\STATE Update $\share{r}$ of $\Replica{j}{r}$ in $\SList$.
%				\ENDIF
%
%				\IF{$a = l$}
%					\STATE Append $\Replica{j}{r}$ to list $\DList$.
%				\ENDIF
%			\ENDWHILE
%		\ENDFOR
%		\STATE {\bf return} $\DList$.
%	\ENDFUNC
%	\SPACE
%
%	\FUNC{transmit}{caller's identifier: $l$, list: $\DList$}
%		\FOR{$r$ : replicas in $\DList$}
%			\STATE $\Replica{j}{r} :=$ receiver replica with share $\share{r}$.
%			\IF{$\share{r} > \share{l}$}
%				\STATE Extract $\share{l}$ messages from $\Sbuf{l}$.
%			\ELSE
%				\STATE Extract $\share{r}$ messages from $\Sbuf{l}$.
%			\ENDIF
%			\STATE Send extracted messages to $\Replica{j}{r}$.
%		\ENDFOR
%	\ENDFUNC
%    \end{myprotocol}
%    \caption{Sharewise Scheduler protocol to identify the message receivers for each caller.}
%    \label{func:sws}
%\end{figure}


 





%{\bf Data Structures.} 
%\nc{I wonder if for simplicity, we would want to describe Scrooge without shares (so that we can keep the notation simple), and then in a second section "refine" it to include shares and include the scheduling? }
%To lay down \Scrooge{} protocol, in the remaining section, we assume that \RSM{s} $\SMR{i}$ and $\SMR{j}$ have access to a 
%steady stream of committed messages that they want to communicate.
%Let $\SSet{i}$ be the set of all messages to be sent by $i$-th \RSM{} $\SMR{i}$, such that:
%\begin{equation*}
%\SSet{i} = \{\SignMessage{m, 1}{\Qusign{i}},  \SignMessage{m, 2}{\Qusign{i}}, ... , \SignMessage{m, \Seqn}{\Qusign{i}}, ... \} 
%\end{equation*}
%%Here, $\SignMessage{m, \Seqn}{\Qusign{i}}$ represents data $m$ committed at sequence number $\Seqn$ by a quorum of replicas in \RSM{} $\SMR{i}$.
%For the sake of explanation, we assume that all the sequence numbers are monotonically increasing and 
%there is no gap in the ordered list of sequence numbers.

%In Section~\ref{s:prelim}, we stated that each replica in \RSM{} $\SMR{i}$ is assigned two identifiers:
%\RSM{} identifier and share identifier.
%If all the replicas have equal share, then $\n{i} = \ts{i}$ and both the identifiers are same.
%We use these identifiers to determine which replica should send which message.
%To do so, we require each replica to maintain several data-structures, which we define next.
%Assume, $l$-th replica $\Replica{i}{l}$ of \RSM{} $\SMR{i}$ has share $\share{l}$ and 
%$\SID{l}$ and $\SID{l-1}$ be the share identifiers of replicas $\Replica{i}{l}$ and $\Replica{i}{(l-1)}$.
%
%\begin{itemize}[wide]
%\item $\Sbuf{l} = \{\SignMessage{m, k}{\Qusign{i}} ~|~ k ~\equiv q \pmod{t_i} ~\wedge ~q \in (\SID{l-1}, \SID{l}] ~\wedge  ~\SignMessage{m, k}{\Qusign{i}} \in \SSet{i} \}$, the set of messages to be sent by $\Replica{i}{l}$, maintained as a queue.
%
%\item $\Hbuf{l} = \SSet{i} - \Sbuf{l}$, the remaining set of messages.
%
%\item $\Rbuf{l} = \{\SignMessage{m, k}{\Qusign{j}} ~|~ j \neq i ~\wedge ~\SignMessage{m, k}{\Qusign{j}} \in \SSet{j} \}$, the messages received from \RSM{} $\SMR{j}$.
%
%\item $\SAck{l} = \{\Ack{k} ~|~ \SignMessage{m, k}{\Qusign{j}} \in \Rbuf{l} \}$, the acknowledgments for messages received from \RSM{} $\SMR{j}$.
%
%\end{itemize}
%%
%\nc{The notion feels very complicated and very protocol heavy when what we're saying is that we're keeping a queue (window) of messages to send, a set of messages received, and a running total of acknowledgements. I suspect we'll want to lighten this up a little bit and make this less formal.} We also require each replica in \RSM{} $\SMR{i}$ to count the number of acknowledgments it has received for 
%each message in the set $\SSet{i}$ from the replicas in \RSM{} $\SMR{j}$. 
%It maintains a map $\RAck{l}{}$ for this purpose. 
%The following example illustrates the use of data-structures $\Sbuf{}$ and $\Hbuf{}$ in practice.


%\begin{example}\label{ex:rep-send}
%Assume two \RSM{s} $\SMR{i}$ and $\SMR{j}$ have $4$ replicas each: 
%$\Replica{i}{1}$, $\Replica{i}{2}$, $\Replica{i}{3}$, and $\Replica{i}{4}$ at $\SMR{i}$, and 
%$\Replica{j}{1}$, $\Replica{j}{2}$, $\Replica{j}{3}$, and $\Replica{j}{4}$ at $\SMR{j}$.
%Say the replicas of \RSM{} $\SMR{i}$ plan to send a series of ordered messages, starting with sequence number $1$. 
%So, the data-structures $\Sbuf{}$ and $\Hbuf{}$ for each replica in $\SMR{i}$ looks as follows:
%$\Sbuf{1} = \{1,5,9,...\}$ and $\Hbuf{1} = \{2,3,4,6,7,8,...\}$, 
%$\Sbuf{2} = \{2,6,10,...\}$ and $\Hbuf{2} = \{1,3,4,5,7,8,...\}$, 
%$\Sbuf{3} = \{3,7,11,...\}$ and $\Hbuf{3} = \{1,2,4,5,6,8,...\}$, and
%$\Sbuf{4} = \{4,8,12,...\}$ and $\Hbuf{4} = \{1,2,3,5,6,7,...\}$.
%\end{example}



%The replicas are sorted on the value of their shares; 
%if two replicas have equal shares, then order the replicas on basis of their identifiers.
%Each replica $\Replica{i}{l}$ of the sending \RSM{} $\SMR{i}$ scans the list $\SList$
%and independently identifies the correct receiver for every replica in $\SMR{i}$.
%The first replica $\Replica{i}{l}$ ($l=0$) of $\SMR{i}$ selects from $\SList$ the replica with the smallest share. 
%Let $\Replica{j}{r}$ be the selected replica and $\share{l}$ and $\share{r}$ be the shares of $\Replica{i}{l}$ and $\Replica{j}{r}$, respectively. 
%If $\share{l} \ge \share{r}$, replica $\Replica{i}{l}$ dequeues $\share{r}$ messages from its $\Sbuf{l}$,
%sends these messages to $\Replica{j}{r}$, 
%removes $\Replica{j}{r}$ from $\SList{}$,
%temporarily reduces $\share{l}$ by $\share{r}$, and appends $\Replica{j}{r}$ to $\SList{}$ with the 
%updated share of $\Replica{j}{r}$ being the sum of total share $\ts{i}$ and $\share{r}$.
%Next, replica $\Replica{i}{l}$ selects the next replica in the sorted list and continues this process until 
%$\share{l}$ is equal to zero.
%If $\share{l} < \share{r}$, replica $\Replica{i}{l}$ dequeues $\share{l}$ messages from its $\Sbuf{l}$, 
%sends these messages to $\Replica{j}{r}$, and temporarily reduces the share $\share{r}$ by $\share{l}$ and sets $\share{l} = 0$.
%Once the share of replica $l=0$ is zero, we continue this process for the replica $l=1$ on the updated list. 

%To identify the correct destination, we design a pairwise round-robin algorithm; 
%$\Replica{i}{l}$ sends the message to replica $\Replica{j}{r}$ of \RSM{} $\SMR{j}$, 
%where $r$ represents the communication round and $r = (l+r) \bmod \n{j} ~\wedge ~r \in [1,\n{j}]$.
%Specifically, in each communication round, each replica $\Replica{i}{l}$ 
%sends a message to a replica of the other \RSM{}; the destination replica varies per round.
%A key advantage of switching destination is to prevent honest replicas to be stuck with byzantine replicas.





%\Scrooge{} requires each honest replica to acknowledge the receipt of a valid message. 
%When a replica $\Replica{i}{l}$ in \RSM{} $\SMR{i}$ receives a message with sequence number $\Seqn$ 
%from the \RSM{} $\SMR{j}$, 
%it creates an acknowledgment $\Ack{k}$ in set $\SAck{l}$.
%
%
%We visualize $\Rbuf{}$ as an array, which stores a copy of received message from the other cluster, 
%indexed by the sequence number.
%We also require replicas to acknowledge (\Name{Ack}) messages they have received from the other cluster. 
%But, sending $\n{}$ \Name{Ack} messages for each received messaged is expensive, so we make replicas send 
%cumulative acknowledgment messages, which help to acknowledge receipt of multiple messages in a shot. 
%In this draft, when a replica sends $\Ack{k}$, it implies that this replica has received all the messages 
%with sequence number less than or equal to $k$.
%Next, we discuss the protocol steps.



%{\bf Complexity.}
%In the normal-case, when there are no failures, every replica in either \RSM{} will send and receive each message.
%Each receiver will get a message either from a replica in the other \RSM{} or through broadcast from a replica in its \RSM{}. 
%So, {\em one} message delay to send a message across \RSM{}, and {\em two} message delays to send a message to all the replicas in a \RSM{}.
%However, the sender cannot remove a message from its $\Sbuf{}$ or $\Hbuf{}$ unless it receives $\f{}+1$ cumulative $\Ack{}$ messages (majority acknowledged) 
%from distinct replicas.
%As cumulative acknowledgments imply  receipt of a sequence of messages, so at steady state {\em two} communications across \RSM{} 
%per message.








==> eval.tex <==

\begin{figure}[t]
    %\vspace{-6mm}
    \centering
     \begin{subfigure}[b]{0.24\columnwidth}
         \centering
         \includegraphics[width=0.745\textwidth]{one-shot.pdf}
         \caption{\OTO{}}
         \label{fig:one-to-one}
     \end{subfigure}%
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{leader-leader.pdf}
         \caption{\LL{}}
         \label{fig:leader-to-leader}
     \end{subfigure}%
     \begin{subfigure}[b]{0.24\columnwidth}
         \centering
         \includegraphics[width=0.745\textwidth]{all-to-all.pdf}
         \caption{\ATA{}}
         \label{fig:all-to-all}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         \includegraphics[width=.75\textwidth]{kafka.pdf}
         \caption{\Kafka{}}
         \label{fig:kafka}
     \end{subfigure}%
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{geobft.pdf}
         \caption{\OTF{}}
         \label{fig:geobft}
     \end{subfigure}%
     \begin{subfigure}[b]{0.25\columnwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{scrooge.pdf}
         \caption{\Scrooge{}}
         \label{fig:scrooge}
     \end{subfigure}
    \caption{\CCC{} baseline summary.}
    \label{fig:c3b-protocols}
\end{figure}

\begin{figure*}[!th]
        %\vspace{-5mm}
    \centering
    \setlength{\tabcolsep}{1pt}
    \scalebox{0.6}{\ref{mainlegendN}}\\[5pt]
    \begin{tabular}{cccc}
    \graphFMsgB & \graphFMsgMB  & \graphFFTP  & \graphFSTP    %& \scalebox{0.6}{\ref{mainlegend}}
    \end{tabular}
    \caption{Throughput of \CCC{} protocols as a function of network size and message size}
    \label{fig:file-non-fail}
    \vspace{-6mm}
\end{figure*}

\section{Evaluation}
\label{s:eval}
\Scrooge{} seeks to offer good performance in the common-case, while remaining robust to faults when failures do arise. We aim to answer the following three questions.
\begin{enumerate}[nosep,wide]
    \item How does \Scrooge{} perform without failures? (\S\ref{ss:file})
    \item Is \Scrooge{}'s performance robust to failures? (\S\ref{ss:perf-failures})
    \item Can \Scrooge{} be used by real applications (\S\ref{ss:real-world})?
    %\CFT{} and \BFT{} RSMs such as Algorand, PBFT, and Raft? 
\end{enumerate}

% We will compare \Scrooge{} against five other protocols, three of which are basic baseline cross-RSM protocol implementations and two of which are real-world communication protocols. We will also run \Scrooge{} in real-world applications like a blockchain wallet exchange and a disaster recovery replication scenario. \mm{Don't love this intro - want to give an overview of the eval, but not sure if it's even necessary...}
% We describe our broad experimental setup, methodology, and implementation details below.

\par \textbf{Implementation} We implemented \Scrooge{} in $\approx$ 4500 lines of C++20 code with Google Protobuf v$3.10.0$ for serialization and NNG v$1.5.2$ for networking.
\Scrooge{} is designed to be a plug-and-play library that can be easily integrated with existing \RSM{s}.
%As stated in Figure~\ref{fig:end-flow}, we assume each \RSM{} 
%interfaces with the \CCC{} protocol to transmit messages. 
%In each \RSM{}, we introduce two additional threads to enable the RSM to forward messages to \Scrooge{}, and receive \quack{}s}.  
%We ensure that the \RSM{} waits to receive a \quack{} for a forwarded message before responding to the client. 

\par \textbf{\CCC{} Baselines.} We evaluate \Scrooge{} against five other comparable protocols (Figure~\ref{fig:c3b-protocols}), which we implement as part of the same framework.
%\mk{Figure 7(f) looks very similar to LL. I don't have a suggestion for how to improve it (maybe multiple dotted arrows?), but this omits all the subtle (and important) differences between the two designs. Maybe simply point the arrow to the second replica, so it's more clear that this isn't a leader.}
\begin{enumerate}[nosep,wide]
    \item {\bf One-Shot (\OTO{})}: In OST, a message is sent by a single sender to a single receiver. 
    \OTO{} is \textit{only} meant as a performance upper-bound. It does not satisfy \CCC{} as message delivery cannot be guaranteed.   
    \item {\bf All-To-All (\ATA{})}: In \ATA{}, every replica in the sending \RSM{} sends all messages to all receiving replicas ($O(\n{s}\times \n{r})$ message complexity). As in \Scrooge{}, every correct receiver is guaranteed to eventually receive the message.
    %Unlike \Scrooge{}, \ATA{} provides no feedback to the sender on when this message will be received by all correct nodes.
    % TCP Acks guarantee this^
    \item {\bf Leader-To-Leader (\LL{})}: The leader of the sending RSM sends a message to the leader of the receiving RSM, who then internally broadcasts the message. Though \LL{} achieves good performance in the failure-free case, this protocol alone does not guarantee eventual delivery when leaders are faulty. %It also does not handle weighted replicas. 
    \item {\bf \Kafka{}}: 
    Apache \Kafka{} is the de-facto industry-standard for exchanging data between services~\cite{kreps2011kafka}. Producers write data to a Kafka cluster, while consumers read data from it. Kafka, internally, uses Raft~\cite{raft} to reliably disseminate messages to consumers. We use Kafka 2.13-3.7.0.
    \item {\bf \OTF{}}: GeoBFT \cite{geobft} targets geo-replicated RSMs and breaks down an RSM into a set of sub-RSMs. Much like \LL, GeoBFT's cross-cluster cluster communication protocol, \OTF{}, has the leader of the sender \RSM{} send  its messages to at least $\uf{r}+1$ receiver \RSM{} replicas. Each receiver then internally broadcast these messages. When the leader is faulty, replicas timeout and request a resend. \OTF{} thus guarantees eventual delivery after at most $\uf{s}+1$ resends in the worst-case (for  $O(\uf{r} * \uf{s})$ total messages). 
\end{enumerate}
%The first three protocols listed above (OST, ATA, and LL) are considered "basline" implementations, as they are meant to give us a reference by which we can measure Scrooge's maximal theoretic throughput. The latter two protocols (\Kafka{}, and GeoBFT) are real-world protocols which we benchmark against to demonstrate that our throughput is better than the current state-of-the-art while still keeping our message overhead low. Reference Figure~\ref{fig:prot-comparison} to see a summary of the differences between these protocols. 
%\mm{This should go in the related work: We do not consider the recently proposed Cross-Chain Interoperability Protocol (CCIP)~\cite{ccip}
%as it uses a centralized risk management network, which developers cannot access. So, we cannot measure the performance of CCIP.}i


\par \textbf{\RSM{s}.} We consider four representative RSMs.
\begin{enumerate}[nosep,wide]
    \item \textbf{\File{}}: An in-memory file from which a replica can generate committed messages infinitely fast. This baseline artificially saturates \CCC{} protocols.
    \item \textbf{\Raft{}~\cite{etcd-raft}}: A widely used CFT \RSM{}, used in services like Kubernetes Cluster. We run Etcd's \Raft{} version v3.0. 
    \item \textbf{\ResDB{}~\cite{resilientdb}}: A high performance implementation of \textit{PBFT}~\cite{pbftj}, a well-known representative BFT protocol.
    \item \textbf{\Algo{}~\cite{algorand}}: A popular \PoS{} blockchain protocol, where committee participation is driven by the amount of stake a participant has in the system~\cite{algorand}. 
\end{enumerate}

\par {\bf Experimental Setup.}
We deploy up to $45$ GCP c2-standard-8 nodes 
(Intel Cascade Lake, $8$vCPU, $32$ GiB RAM, 15 GBits/s). 
Each experiment runs for $180$ seconds ($30$ second warmup/cool down). All experiments run \Scrooge{} with a $\phi$-list of \si{200}{k} and $256$ bits for 0.1kB and \si{1}{MB} batches, respectively (best results for our specific network setup). 
We tune the batch size of each \RSM{} to ensure good throughput.  We further assume that RSMs forward all messages to the other RSM, as this represents a worst-case scenario for \Scrooge{}. As is standard~\cite{hotstuff,quepaxa,basil,kauri}, replicated operations in our experiments are no-ops only, which ensures that the bottleneck is either \RSM{} or \Scrooge{}.

\par {\bf Metrics.}
We consider \textit{\RSM{} throughput}, the number of consensus invocations completed at an \RSM{} per unit of time,
as well as \textit{\CCC{} throughput}, the number of completed \CCC{} invocations per unit of time.
For \Scrooge{}, \CCC{} throughput refers to the number of unique \quack{s} per unit of time.
When baselines, like \OTO{}, do not acknowledge received messages,
we calculate \CCC{} throughput as the number of unique messages sent from sender \RSM{} to receiver \RSM{}. 

%{\bf Metrics.} We primarily study throughput in this evaluation section. We analyze the affects of \RSM{} network size and message size on throughput, testing our scalability and our resource utilization, as well as our ability to handle different payload sizes. We also conduct experiments measuring throughput when the \RSM{s} are Geo-replicated, which allows us to test performance in a lower-bandwidth setting. In our experiments, we measure throughput at the respective \CCC{} protocol and their corresponding \RSM{s} application. \RSM{} throughput is the number of consensus invocations completed at an \RSM{} per unit of time, and \CCC{} throughput is the number of completed \CCC{} invocations per unit of time. For \Scrooge{}, \CCC{} throughput refers to the number of unique \quack{s} per unit of time at a correct replica. As all other baselines do not acknowledge received messages, \CCC{} throughput for these protocols is equal to the number of unique messages sent from sender \RSM{} to receiver \RSM{} per unit time. While all but \OTO{} and \LL{} provide eventual delivery implement \CCC{} and thus guarantees eventual delivery, we cannot detect when delivery actually takes place. \mm{Need to include discussion of latency somehow: For similar reasons, we do not plot latency.}
%

%\begin{figure}
%        %\vspace{-5mm}
%    \centering
%    \setlength{\tabcolsep}{1pt}
%    %\scalebox{0.6}{\ref{mainlegend}}\\[5pt]
%    \begin{tabular}{cc@{\quad}cc}
%    \graphFMsgB & \graphFMsgMB  \\
%    \graphFFTP  & \graphFSTP    \\
%    \graphGEO   & \scalebox{0.6}{\ref{mainlegend}}
%    \end{tabular}
%    
%    \caption{Throughput of \CCC{} protocols as a function of network size and message size.}
%    \label{fig:file-non-fail}
%\end{figure}
\iffalse
\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|} \hline
            & \OTO{}    & \LL{}     & \ATA{}    & \Kafka{}  & \OTF{}    & \Scrooge{}    \\ \hline 
  \CCC{}    & \xmark    & \cmark    & \cmark    & \cmark    & \cmark    & \cmark        \\ \hline
  Byzantine Resilient & \xmark    & \cmark    & \cmark    & \xmark    & \cmark    & \cmark        \\ \hline
  Asynchronous & \xmark    & \xmark    & \xmark    & \xmark    & \xmark    & \cmark        \\ \hline
  Sender \RSM{} knows if message delivered  & \xmark    & \xmark    & \cmark    & \cmark    & \xmark    & \cmark        \\ \hline
  Dynamic Scheduling for weighted \RSM{s}    & \xmark    & \xmark    & \xmark    & \xmark    & \xmark    & \cmark        \\ \hline
\end{tabular}
\caption{\sg{Comparing different communication protocols.}}
\label{fig:prot-comparison}
\end{figure}
\fi

\subsection{Scalability}
\label{ss:file}


% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \begin{tabular}{|c|c|} 
%     OST & 1 \\
%     LL & O(n) + O(n) \\
%     ATA & O(n^2)
% \end{tabular}
%     \label{fig:enter-label}
% \end{figure}

% We consider five comparison protocols, three of which are basic communication protocols (\OTO{}, \LL{}, and \ATA{}) and 
% two which are real-world communication protocols (\Kafka{} and \OTF{}). We describe each protocol next:

Our first set of experiments aim to stress test the six \CCC{} protocols (\Scrooge{}, \ATA{}, \LL{}, \OTO{}, \OTF{} and Kafka). We use the ``infinitely fast'' File RSM to saturate all \CCC{} implementations. In all cases, we include the \OTO{} line as the upper-bound of our networking implementation.

{\bf Varying number of replicas in each \RSM{}.}
We first consider the relative performance of \Scrooge{} over \ATA{} as a function of the network size.
We fix the message size to \SI{0.1}{kB} and \SI{1}{MB} and increase the number of replicas in each \RSM{} from $4$ to $19$ (Figure~\ref{fig:file-non-fail}(i)-(ii)). For small network sizes, \Scrooge{} outperforms \ATA{} by a factor of $2.5\times$ (small messages) and $3.2\times$ (large messages). 
This performance benefit of \Scrooge{} increases
in the larger network ($6.6\times$ and $12.1\times$). \Scrooge{} sends only a linear number of messages whereas \ATA{} must send/receive a quadratic number of messages.
Like \Scrooge{}, \LL{} and \OTF{} send a linear number of copies of each message, but quickly bottleneck at the leader (that needs to send every message).
Thus, \Scrooge{} is faster than \LL{} and \OTF{} by $1.6\times$ and $1.9\times$ for small network sizes and $4.4\times$ and $4.8\times$ for large network sizes, respectively (on small messages).
%\nc{network size? can you make sure that the sentence flows with the text?}
%\nc{respectively 19 and how many for Geo?}.
%The relative gains for large network sizes and large messages are comparatively smaller as \Scrooge{} becomes network-bottlenecked.
\OTO{}'s performance, as expected, increases with network size as increasing the number of replicas increases the number of parallel messages.
Kafka performs significantly worse in all cases as it internally runs consensus.
\par{\bf Varying Message Size.}
In Figure~\ref{fig:file-non-fail}(iii)-(iv), we fix the size of each \RSM{} to $n=4$ (small) and $n=19$ replicas (large)
and increase the message size from \SI{0.1}{kB} to \SI{1}{MB}.  We confirm the expected results: the performance of each \CCC{} implementation drops as a linear function of message size. Note that \Scrooge{} performs relatively better than other protocols for large message sizes  as larger sizes hide the moderate compute overheads introduced by the system. 
For instance, on a large network \Scrooge{} performs $12.1\times$, $12.7\times$, and $12.5\times$ better than \ATA{}, \LL{}, and \OTF{}, respectively, for large messages, compared to $6.6\times$, $4.4\times$, and $4.9\times$ when messages are small.  
%\sg{In contrast, on a large network \LL{} and \OTF{} perform $2\%$ and $1\%$ better than \ATA{} for large messages, 
%compared to $50\%$ and $45\%$ when messages are small.}\nc{not sure we need this given it's not in relation to scrooge}



\iffalse
\subsubsection{Real-World Implementations}
[TODO - GeoBFT message overhead, Kafka scaling issues. INSERT GRAPH HERE]
\nc{Don't understand what this section is for?}
\fi

\subsection{Performance under failures}
\label{ss:perf-failures}
We first consider crash failures before investigating the impact of Byzantine failures.

\begin{figure*}
        %\vspace{-5mm}
    \centering
    \setlength{\tabcolsep}{1pt}
    \scalebox{0.6}{\ref{mainlegend3}} \quad
    \scalebox{0.6}{\ref{mainlegend5}} \quad 
    \scalebox{0.6}{\ref{mainlegend4}} \\[5pt]
    \begin{tabular}{ccc}
    \graphFail    & \graphBPhiList  &   \graphBAcking 
    \end{tabular}
    \caption{Effects of Failures on \Scrooge{}.}
    \label{fig:byz-failures}
    \vspace{-6mm}
\end{figure*}
\par \textbf{Crash Failures.} 
We conduct a simple experiment in which we randomly crash 33\% of the replicas in each RSM (Figure~\ref{fig:byz-failures}(i)). We consider a message size of \SI{1}{MB}  (results are similar for smaller messages) and set the $\phi$-list size as $512$. 
\Scrooge{}'s performance drops by a factor of $32.9\%$. This is expected:
\Scrooge{}, by default, fully maxes out links with "useful" information (a single message sent). Removing a third of the links thus removes a third of the available bandwidth. 
Nonetheless, \Scrooge{} continues to outperform \ATA{} by $2.7\times$ on small networks (size $4$), and up to $8.9\times$ on larger networks.  \ATA{}'s performance does not degrade during failures: \ATA{}, in effect, preemptively assumes that all replicas have failed and thus always has all replicas send all messages all the time. While \Scrooge{}'s performance may converge to that of \ATA{} when failures increase, it will never become worse than \ATA{}.

\par \textbf{Byzantine Failures}
Next, we consider the impact of Byzantine failures in the system. 
There are four main types of attacks. Malicious nodes can (1) send invalid, uncommitted messages, 
(2) collude to drop long sequences of message $\uf{s}+\uf{r}+1$ times, 
(3) selectively drop messages, and (4) send incorrect acknowledgements. The first attack amounts to a DDOS attack (as correct replicas will discard invalid messages) and thus out of scope. \Scrooge{} defends against the second attack by assigning node IDs using a verified source of randomness.
We focus on the last two scenarios.


\begin{enumerate}[nosep,wide]
    \item \textbf{Impact of $\phi$-list scaling on Byzantine failures.}
    $\phi$-lists bound the possible performance drop from malicious nodes selectively dropping messages.
    We again assume $33\%$ faulty replicas in both RSMs (Figure~\ref{fig:byz-failures}(ii)), this time Byzantine. We consider a message size of \SI{1}{MB}. 
  %  This experiment aims to illustrate the impact of $\phi$-list size on the performance of \Scrooge{}.
 %   In contrast to the common %expectation that an increase in the $\phi$-list size should decrease the performance of the \Scrooge{}, 
    Our results illustrate that the larger $\phi$-list size helps \Scrooge{} quickly recover from Byzantine failures.
    This is despite the larger $\phi$-list increasing message sizes.
    We observe that a $\phi$-list size of $256$ is optimal for recovering from the $33\%$ Byzantine attacks. As the network gets larger, the time it takes to complete a full broadcast gets longer, which increases latency to confirm a delivery. Thus, more messages can be dropped before we can detect that they are not dropped, hence the larger $\phi$-list.
    \item \textbf{Sending incorrect acks.} 
    Malicious nodes can choose to lie in their acknowledgements. We simulate this behaviour in Figure~\ref{fig:byz-failures}(iii) by having malicious nodes send acks for overly high sequence numbers (Scrooge-Inf), overly low ones (Scrooge-0) or offset by $\phi$ (Scrooge-Delay).
    We find that this behaviour is much less harmful than simply crashing.  
    Correct nodes wait for a quorum of $\uf{r}+1$ matching acks in order to consider the message delivered, and thus already assume that $\uf{}$ of those acks will be lies. 
    Lying about an ack thus only temporarily delays the formation of a quorum.  
    %This is in line with Scrooge's ethos: much like Aardvark~\cite{}, Scrooge's primary design requirement is not just performance but robustness to failures.
    %\item \textbf{Colluding to repeatedly drop messages.} Malicious nodes can try to influence the choice of sender-receiver pairs to maximize the number of times these pairings include a faulty node. In the worst case, this strategy could result in \Scrooge{} resending messages $u_{sender} + u_{receiver}$ times, causing throughput to crater (\nc{Add result}). In practice, \Scrooge{} ensures that this scenario cannot happen, except with low probability. Node IDs are assigned by \Scrooge{} using  using a verifiable source of randomness, thus precluding any collision. \nc{TODO: add results}.
    %The use of $\phi$-lists further ensures that dropped messages can be retransmitted quickly and in parallel. \nc{Add result}
    %However, Theorem 1 shows that \Scrooge{}, with high probability, will never drop a message more than 72 times even if $u_{sender}+u_{receiver}$ is unbounded, minimizing Byzantine influence.
\end{enumerate}
%[INSERT GRAPHS AND EXPLANATION OF EXPERIMENTS HERE, also add in "Baseline" line to graph and describe it in the text]
%The design of \Scrooge{} has been greatly influenced by the lessons of Aardvark \cite{aardvark}. True to Aardvark's spirit, \Scrooge{} does not have an optimistic path that defers work to the failure path (like Zyzzyva \cite{zyzzyva} and other speculative approaches do). Instead, we are pessimistic and always include sufficient information ($\phi$-lists) to retransmit missing messages. Our evaluation shows we perform well even with the maximum number of failures (Figure~\ref{fig:file-stake-fail}(ii)). As \Scrooge{} fully leverages the bandwidth of all nodes, killing a node naturally comes with a performance cost; this is fundamental. Nonetheless, in the failure case our performance still shines (6.6x vs ATA).
%




% message_size,latency,throughput,strategy,local_network_size,foreign_network_size
% 1000000,0,27.883312317815374,All-to-All,4,4
% 1000000,0,15.900000265000221,All-to-All,7,7
% 1000000,0,10.96667416056202,All-to-All,10,10
% 1000000,0,0.033333346666672,All-to-All,13,13
% 1000000,0,6.483335269446867,All-to-All,16,16
% 1000000,0,5.249999740000131,All-to-All,19,19
% 1000000,0,105.69999656000023,Scrooge k=64+ resends,4,4
% 1000000,0,104.69998509334587,Scrooge k=64+ resends,7,7
% 1000000,0,76.16668948779224,Scrooge k=64+ resends,10,10
% 1000000,0,89.3000304216826,Scrooge k=64+ resends,13,13
% 1000000,0,48.43330666669511,Scrooge k=64+ resends,16,16
% 1000000,0,44.01666936891273,Scrooge k=64+ resends,19,19


\subsection{Impact of Geo-replication and Stake}
In Figure~\ref{fig:file-stake-fail}(i), we run geo-replicated experiments by deploying one \RSM{} in US West and other \RSM{} in Hong Kong
(cross-region bandwidth, \textit{pair-wise} is \SI{170}{Mbits\per\sec}, ping time \SI{133}{ms}). We fix the message size to \SI{1}{MB} and increase \RSM{} size from $4$ to $19$. The lower bandwidth across \RSM{}s disproportionally affects \ATA{}, \LL{}, and \OTF{}.
\Scrooge{} outperforms \ATA{}, %\LL{}, and \OTF{} 
by $12\times$ 
%, $X\times$, and $Y\times$
(for network size $4$) and $44\times$, %$Z\times$, and $E\times$ 
(for network size $19$). Somewhat counter-intuitively, the performance of both \Scrooge{} and \OTO{} increase as a function of network size: increasing the number of receivers gives senders access to more bandwidth. \Scrooge{} intentionally has its senders send to multiple receivers and thus (artificially) outperforms \OTO{}, which fixes unique sender-receiver pairs. 



Next, we ask how well \Scrooge{} performs when (1) stake grows large and (2) when stake distribution is unequal. We fix the message size to \SI{1}{MB}. All nodes are bandwidth-bottlenecked.
To answer the first question, consider a setup in which one \RSM{} has stake $\n{}$ and the other has stake $\n{} * 1000$; stake itself is divided equally amongst replicas (\Scrooge-Large). We find that \Scrooge-Large has identical throughput to the equal stake case. This is expected, as \Scrooge{}'s apportionment and LCM logic will reduce the message sending/receiving pattern back to the fully equal stake case.
Next, we look at unequal stake distribution. 
Consider (i) two \RSM{s} where the stake of each replica is different;
each replica has stake equal to its logical identifier ($\Replica{i}{1}$ stake = 1, $\Replica{i}{2}$ stake = 2, ...). (\Scrooge-Graded) (ii) two \RSM{s} where one replica holds $50\%$ stake and the remaining $50\%$ stake is divided among all the other replicas (\Scrooge{}-Unfair). All replicas continue to have equal computing power and bandwidth.
Unequal stake \textit{combined with equal bandwidth} causes \Scrooge's performance to drop (by $33\%$ for \Scrooge-Graded and $87\%$ for \Scrooge-Unfair) as the communication load is no longer balanced across replicas. This effect is especially pronounced in \Scrooge-Unfair where the one replica with $50\%$
has to  both send 50\% of the messages to the other RSM as well as receive messages from 50\% of the other \RSM{}'s replicas. In practice, nodes with higher stake are more powerful than their low-stake counterparts, thus side-stepping this issue. 
%We emulate this in \Scrooge{}-Fair, where we artificially bound the replicas with low stake to 1Gbits/s using TC~\cite{tc}, giving only the trusted node its full 16Gbit/s bandwidth. 

\iffalse
\subsection{Impact of stake}
\label{ss:stake}
Next, we ask: 1) how well does \Scrooge{} perform when stake grows large.
 (2) when stake distribution is unequal.
We fix the message size to \SI{1}{MB}. 
To simulate the practical reality of nodes with differing trust having different compute/bandwidth resources available, we artificially restrict the bandwidth of each node using TC~\cite{tc} to 1Gb/s. 
All nodes are bandwidth-bottlenecked.

To answer the first question, consider a setup in which one \RSM{} has stake $\n{}$ and the other has stake $\n{} * 1000$; stake itself is divided equally amongst replicas (\Scrooge-Large). We find that \Scrooge-Large has identical throughput to the equal stake case. This is expected, as \Scrooge{}'s apportionment and LCM logic will reduce the message sending/receiving pattern back to the fully equal stake case.

Next, we look at unequal stake distribution. 
Consider (i) two \RSM{s} where the stake of each replica is different;
each replica has stake equal to its logical identifier ($\Replica{i}{1}$ stake = 1, $\Replica{i}{2}$ stake = 2, ...). (\Scrooge-Graded) (ii) two \RSM{s} where one replica holds $50\%$ stake and the remaining $50\%$ stake is divided among all the other replicas. All replicas continue to have equal computing power and bandwidth (\Scrooge{}-Fair) . (iii) 
Two \RSM{s} where one replica holds $50\%$ stake and the remaining $50\%$ stake is divided among all the other replicas, but where the node with $50\%$ stake has 10x the bandwidth of less important nodes (\Scrooge{}-Unfair) \nc{Micah suggested renaming. Maybe to Equal/Unequal?}. 
Unequal stake \textit{combined with equal compute} causes \Scrooge's performance to drop (by $33\%$ for \Scrooge-Graded and $87\%$ for \Scrooge-Unfair) as the communication load is no longer balanced across replicas. This effect is especially pronounced in \Scrooge-Unfair where the one replica with $50\%$
has to  both send 50\% of the messages to the other RSM as well as receive messages from 50\% of the other \RSM{}'s replicas. If we artificially give the high trust node 10x the bandwidth of the other nodes (using TC~\cite{tc}), we see no significant drop in performance over an equal stake setting as the high trust node has sufficient bandwidth to handle the additional load (\Scrooge{}-fair); the stake logic itself adds little overhead to \Scrooge{}.
\fi

\subsection{Case Study: \RSM{}-to-\RSM{} in the Wild}
\label{ss:real-world}
Finally, we describe and evaluate four real-world use-cases for which \Scrooge{} can facilitate communication (Figure~\ref{fig:systems}).

{\bf (1) Disaster Tolerance (DT).}
Disaster tolerance requires mirroring RSMs across datacenters to ensure rapid failover in the event of a mass failure. It is commonly done through cross-datacenter Etcd to Etcd mirroring over Kafka. Using this specific setup, we achieve $\approx$6,211 tx/sec with two Etcd instances and a Kafka cluster located in zone us-central1-a. We run a similar DT scenario using \Scrooge{} to communicate messages between two Etcd's \Raft{} \RSM{s} (version v3.0) in the same zone (C-C), for which we obtained $\approx$68,000 tx/sec. This is in line with Raft's base throughput and a $10.9\times$ throughput increase over using Kafka.

{\bf (2) Decentralized Finance/Blockchain.}
Cross-chain communication is an important prerequisite for greater interoperability~\cite{ccip}.  We consider three scenarios:  1) two \PoS{} \Algo{} chains (A-A), 2) two traditional 
 permissioned PBFT \ResDB~\cite{resilientdb} chains (B-B).
 3) \ResDB{} to \Algo{} interoperability (A-B). 
 \Algo's base throughput with another \Algo~instance is 120 blocks/second. \ResDB's base throughput when communicating with another \ResDB~cluster is $\approx$6000 batches/second (of size \si{5}{kB}). The cross-chain throughput when \Algo~sends to \ResDB~is 135 blocks/second.
 
{\bf (3) Heterogeneous RSMs.}
There are administrative and geographical reasons to run consensus on a first RSM before communicating results to another RSM. Heterogeneous trust is one. We thus test \CFT{} to \BFT{} communication over \Scrooge{} (A-C,B-C).

We find that: (1) \Scrooge{} has minimal impact on the throughput of any of the \RSM{s}, with less than 15\% decrease in throughput in the worst case.
(2) \Scrooge{} successfully handles throughput differences between RSM. The slow Algorand RSM can efficiently communicate with the much faster Raft RSM. 
\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    \scalebox{0.6}{\ref{mainlegendGEO}}
    \scalebox{0.6}{\ref{mainlegend2}}\\[5pt]
    \begin{tabular}{cc}
    \graphGEO   &   \graphFStake 
    \end{tabular}
    \caption{Geo-replication and stake}
    \label{fig:file-stake-fail}
\end{figure}


%\begin{figure}[t]
%    \centering
%    \begin{tabular}{ll}
%    \hspace{-8mm}\klistTp & \hspace{-8mm}\klistLat
%    \end{tabular}
%    \caption{Performance measurements under one failure in each \File{} \RSM{s} as a function of $\phi$-list size.
%    Here, $\n{} = 4$ and message size = \SI{100}{B}.
%   }
%    \label{fig:klist-costs}
%\end{figure}



==> evalEDIT.tex <==
\section{Evaluation}
\label{s:eval}
Our evaluation aims to answer the following three questions.
\begin{enumerate}[nosep,wide]
    \item How does \Scrooge{} perform without failures? (\S\ref{})
    \item Is \Scrooge{} robust to failures? (\S\ref{})
    \item Can \Scrooge{} be used by real applications (\S\ref{})?
    %\CFT{} and \BFT{} RSMs such as Algorand, PBFT, and Raft? 
\end{enumerate}
% We will compare \Scrooge{} against five other protocols, three of which are basic baseline cross-RSM protocol implementations and two of which are real-world communication protocols. We will also run \Scrooge{} in real-world applications like a blockchain wallet exchange and a disaster recovery replication scenario. \mm{Don't love this intro - want to give an overview of the eval, but not sure if it's even necessary...}
% We describe our broad experimental setup, methodology, and implementation details below.

\subsection{Implementation}
 
 We implemented \Scrooge{} in $\approx$ 4500 lines of C++20 code. We use Google's protobuf 
library v$3.10.0$ as our serialization library and NNG v$1.5.2$ for networking.\Scrooge{} is designed to be a plug-and-play library that can be easily integrated with existing \RSM{s}.
As stated in Figure~\ref{fig:end-flow}, we assume each \RSM{} 
interfaces with the \CCC{} protocol to transmit messages. 
In each \RSM{}, we introduce two additional threads to enable the RSM to forward messages to \Scrooge{}, and receive \quack{}s. We ensure that the \RSM{} waits to receive a \quack{} for a forwarded message before responding to the client. 

 
\subsection{Methodology and Setup}

\par \textbf{\CCC{} Baselines} We evaluate Scrooge against five other comparable protocols (three basic and two real-world communication protocols). All custom baselines are implemented as part of the Scrooge framework for a fair comparison. We summarize each baseline in Figure~\ref{fig:c3b-protocols}.
\begin{enumerate}[nosep,wide]
    \item {\bf One-Shot (\OTO{})}: In OST, a message is sent by a single sender to a single receiver. 
    \OTO{} is *only* meant as a performance upper-bound. It does not satisfy \CCC{} as message delivery cannot be guaranteed.   
    \item {\bf All-To-All (\ATA{})}: In \ATA{}, every replica in the sending\RSM{} sends every message to every replica of the receiving \RSM{}. \ATA{} protocol creates and sends $O(\n{1}\times \n{2})$ copies of each message. As in \Scrooge{}, every correct receiver is guaranteed to eventually receive the message. Unlike \Scrooge{}, \ATA{} provides no feedback to the sender on when this message will be received by all correct nodes.
    \item {\bf Leader-To-Leader (\LL{})}: The leader of the sending RSM sends a message to the leader of the receiving RSM, who can internally broadcast the message to nodes in its \RSM{}. Though\LL{} achieves good performance in the failure-free case, this protocol does not guarantee eventual delivery when leaders are faulty. It also does not handle weighted replicas. \OTF{} (below) proposes a leader-to-leader strategy that correctly handles faulty leaders.
    \item {\bf \Kafka{}}: 
    Apache \Kafka{} is the de-facto industry-standard for exchanging data between services~\cite{confluent}. Producers write data to a Kafka cluster, while consumers read data from it. Kafka, internally, uses a custom Raft~\cite{raft} implementation to reliably disseminate messages to consumers.
    \item {\bf OTF{}}: GeoBFT's \cite{geobft} seeks to improve the performance of geo-replicated RSMs. It does so by breaking down an RSM into a set of sub-RSMs. The cross cluster communication protocol, \OTF{}, has the leader of the sender \RSM{} send  its messages to at least $\uf{r}+1$ replicas in the other \RSM{}. Each receiver then internally broadcast these messages to its \RSM{}. In the case of a faulty sender, replicas timeout, requesting a resend. \OTF{} thus guarantees eventual delivery after at most $\uf{s}+1$ resends in the worst-case. 
\end{enumerate}
%The first three protocols listed above (OST, ATA, and LL) are considered "basline" implementations, as they are meant to give us a reference by which we can measure Scrooge's maximal theoretic throughput. The latter two protocols (\Kafka{}, and GeoBFT) are real-world protocols which we benchmark against to demonstrate that our throughput is better than the current state-of-the-art while still keeping our message overhead low. Reference Figure~\ref{fig:prot-comparison} to see a summary of the differences between these protocols. 
%\mm{This should go in the related work: We do not consider the recently proposed Cross-Chain Interoperability Protocol (CCIP)~\cite{ccip}
%as it uses a centralized risk management network, which developers cannot access. So, we cannot measure the performance of CCIP.}i

\par \textbf{\RSM{} Applications} We consider four different RSM implementations, which we view as representative of the wide-space of consensus protocols.
\begin{enumerate}[nosep,wide]
    \item \textbf{\File{}}: This artificial RSM is an in-memory file from which a replica can generate messages infinitely fast. The \File{} application aims to artificially saturate \CCC{} protocols (replicas can issue requests at an unbounded rate without the overhead of consensus).
    \item \textbf{\Raft{}}: Raft~\cite{etcd-raft} is a widely used and mature crash-fault-tolerant RSM, at the core of many production level services such as Kubernetes Cluster. We runs Etcd's \Raft{} version v3.0. 
    \item \textbf{\ResDB{}}: \ResDB{} is a mature framework~\cite{resilientdb} for implementing high performance BFT protocols. Each \ResDB{} \RSM{} runs \pbft{} consensus~\cite{pbftj} to replicate client requests~\cite{geobft}. PBFT represents the de-facto standard amongst traditional BFT protocols.
    \item \textbf{\Algo{}}:  \Algo{} is a popular \PoS{} blockchain protocol, where committee participation is driven by the amount of stake a participant has in the system~\cite{algorand}. 
\end{enumerate}

\par {\bf Experimental Setup.}
We use Google Cloud to deploy up to $45$ c2-standard-8 nodes 
(x86\_64 architecture, Intel Cascade Lake, $8$vCPU, $4$ cores and $32$ GiB RAM) 
at uc-central-1a (Iowa). For non geo-replicated experiments, the network bandwidth was between $13-17$Gbit/s. \mm{Include network numbers for WAN tests.}
Each experiment runs for $180$ seconds ($30$ second warmup/cool down). We report the average throughput over three runs. All experiments run \Scrooge{} with a $\phi$-list of 1000, which we experimentally verified offers the best performance for our specific network setup. Similary, We tune the batch size of each RSM to ensure good throughput.  We further assume that RSMs forward all messages to the other RSM, as this represents a worst-case scenario for Scrooge. As is standard in the space~\cite{}, replicated operations in our experiments are no-ops only, which ensures that the bottleneck is either RSM or Scrooge, and that overheads cannot be masked by execution.

\par {\bf Metrics.}
In our experiments, we measure throughput at both the \RSM{} and respective \CCC{} protocol.
(1) \RSM{} throughput is the number of consensus invocations completed at an \RSM{} per unit of time
(2) \CCC{} throughput is the number of completed \CCC{} invocations per unit of time.
For \Scrooge{}, \CCC{} throughput refers to the number of unique \quack{s} per unit of time at a correct replica.
When baselines, like \ATA{}, do not acknowledge received messages,
we calculate \CCC{} throughput as the number of unique messages sent from sender \RSM{} to receiver \RSM{} per unit time.
For similar reasons, we do not plot latency. 


%{\bf Metrics.} We primarily study throughput in this evaluation section. We analyze the affects of \RSM{} network size and message size on throughput, testing our scalability and our resource utilization, as well as our ability to handle different payload sizes. We also conduct experiments measuring throughput when the \RSM{s} are Geo-replicated, which allows us to test performance in a lower-bandwidth setting. In our experiments, we measure throughput at the respective \CCC{} protocol and their corresponding \RSM{s} application. \RSM{} throughput is the number of consensus invocations completed at an \RSM{} per unit of time, and \CCC{} throughput is the number of completed \CCC{} invocations per unit of time. For \Scrooge{}, \CCC{} throughput refers to the number of unique \quack{s} per unit of time at a correct replica. As all other baselines do not acknowledge received messages, \CCC{} throughput for these protocols is equal to the number of unique messages sent from sender \RSM{} to receiver \RSM{} per unit time. While all but \OTO{} and \LL{} provide eventual delivery implement \CCC{} and thus guarantees eventual delivery, we cannot detect when delivery actually takes place. \mm{Need to include discussion of latency somehow: For similar reasons, we do not plot latency.}
%

%\begin{figure}
%        %\vspace{-5mm}
%    \centering
%    \setlength{\tabcolsep}{1pt}
%    %\scalebox{0.6}{\ref{mainlegend}}\\[5pt]
%    \begin{tabular}{cc@{\quad}cc}
%    \graphFMsgB & \graphFMsgMB  \\
%    \graphFFTP  & \graphFSTP    \\
%    \graphGEO   & \scalebox{0.6}{\ref{mainlegend}}
%    \end{tabular}
%    
%    \caption{Throughput of \CCC{} protocols as a function of network size and message size.}
%    \label{fig:file-non-fail}
%\end{figure}
\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|} \hline
            & \OTO{}    & \LL{}     & \ATA{}    & \Kafka{}  & \OTF{}    & \Scrooge{}    \\ \hline 
  \CCC{}    & \xmark    & \cmark    & \cmark    & \cmark    & \cmark    & \cmark        \\ \hline
  Byzantine Resilient & \xmark    & \cmark    & \cmark    & \xmark    & \cmark    & \cmark        \\ \hline
  Asynchronous & \xmark    & \xmark    & \xmark    & \xmark    & \xmark    & \cmark        \\ \hline
  Sender \RSM{} knows if message delivered  & \xmark    & \xmark    & \cmark    & \cmark    & \xmark    & \cmark        \\ \hline
  Dynamic Scheduling for weighted \RSM{s}    & \xmark    & \xmark    & \xmark    & \xmark    & \xmark    & \cmark        \\ \hline
\end{tabular}
\caption{\sg{Comparing different communication protocols.}}
\label{fig:prot-comparison}
\end{figure}


\subsection{Scalability}
\label{ss:file}
\begin{figure*}
        %\vspace{-5mm}
    \centering
    \setlength{\tabcolsep}{1pt}
    \scalebox{0.6}{\ref{mainlegend}}\\[5pt]
    \begin{tabular}{ccccc}
    \graphFMsgB & \graphFMsgMB  &   \graphFFTP  & \graphFSTP    &   \graphGEO   %& \scalebox{0.6}{\ref{mainlegend}}
    \end{tabular}
    \caption{Throughput of \CCC{} protocols as a function of network size, message size, and geo-replication.}
    \label{fig:file-non-fail}
\end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \begin{tabular}{|c|c|} 
%     OST & 1 \\
%     LL & O(n) + O(n) \\
%     ATA & O(n^2)
% \end{tabular}
%     \label{fig:enter-label}
% \end{figure}

% We consider five comparison protocols, three of which are basic communication protocols (\OTO{}, \LL{}, and \ATA{}) and 
% two which are real-world communication protocols (\Kafka{} and \OTF{}). We describe each protocol next:

Our first set of experiments aim to stress test the three \nc{five?} \CCC{} protocols (\Scrooge{}, \ATA{} and \OTO{})  
by deploying each protocol between two \File{} \RSM{s}.
In a \File{} \RSM{}, we assume an in-memory file from which one can artificially generate proposals at an "infinite" rate. The goal is to saturate the \CCC{} primitive implementations and identify their peak throughput. In all cases, we include the \OTO{} line as a reference point of what the maximum send/receive rate of our networking implementation is. \OTO{} is strictly an upper-bound as it does not guarantee delivery under failures. 

{\bf Varying number of replicas in each \RSM{}.}
We first consider the relative performance of \Scrooge{} over \ATA{} as a function of the network size.
We fix the message size to \SI{0.1}{kB} and \SI{1}{MB} and increase the number of replicas in each \RSM{} from $4$ to $19$ (Figure~\ref{fig:file-non-fail}(i)-(ii)). For small network sizes, \Scrooge{} outperforms \ATA{} by a factor of $1.84\times$ (small messages) and $3.7\times$ (large messages). 
This performance benefit of \Scrooge{} increases
in the larger network ($8.4\times$ and $13.4\times$). \Scrooge{} sends only a linear number of messages whereas \ATA{} must send/receive quadratic number of messages. 
%The relative gains for large network sizes and large messages are comparatively smaller as \Scrooge{} becomes network-bottlenecked.
\OTO{}'s performance, as expected, increases with network size as increasing the number of replicas increases the number of messages that can be sent in parallel.

{\bf Varying Message Size.}
In Figure~\ref{fig:file-non-fail}(iii)-(iv), we fix the size of each \RSM{} to $n=4$ (small) and $n=19$ replicas (large)
and increase the message size from \SI{0.1}{kB} to \SI{1}{MB}.  We confirm the expected results: the performance of each \CCC{} implementation drops as a linear function of message size. Scrooge outperforms \ATA{} by a factor of $3.25\times$ and $15.3\times$ (respectively for small and large networks) for large message sizes, 
but only outperforms \ATA{} by a factor of $1.84\times$ and $8.4\times$ (respectively for small and large networks) for smaller messages. Larger messages hide the moderate compute overhead introduced by Scrooge; the relative performance gains are thus larger for bigger messages.

{\bf Geo-replication.} 
In Figure~\ref{fig:file-non-fail}(v), we run geo-replicated experiments by deploying one \RSM{} in Iowa and other \RSM{} in Hong Kong. 
The available bandwidth between two replicas in different \RSM{s} is approximately \SI{135}{Mbits\per\sec} and ping time is \SI{163}{m\sec}.
In these experiments, we fix the message size to \SI{1}{MB} and increase the number of replicas in each \RSM{} from $4$ to $19$. The lower bandwidth across \RSM{}s disproportionally affects \ATA{}. 
In this setup, \Scrooge{} outperforms \ATA{} by $9.7\times$ (small network) and $24\times$ (large network). Somewhat counter-intuitively, the performance of both \Scrooge{} and \OTO{} increase as a function of network size: this is because bandwidth is bound to \SI{135}{Mbits\per\sec} 
\textit{per pairwise connection}. Increasing the number of receivers thus gives senders access to more bandwidth. \Scrooge{} intentionally has its senders send to multiple receivers and thus (artificially) outperforms \OTO{}, which selects unique sender-receiver pairs. 

\subsection{Impact of stake}
Next, in Figure~\ref{fig:file-stake-fail}(i), we fix the message size to \SI{1}{MB}
and increase the number of replicas in each \RSM{} from $4$ to $19$.
We answer two questions: (1) how does \Scrooge{} perform when stake grows large, and (2) how does unequal stake affect the performance of \Scrooge{}. To answer these questions, we consider  four scenarios:
(i) Two \RSM{s} where the stake of each replica is different;
each replica has stake equal to its logical identifier ($\Replica{i}{1}$ stake = 1, $\Replica{i}{2}$ stake = 2, ...). (\textit{\Scrooge-Graded})
(ii) One \RSM{} with stake $\n{}$ and other with stake $\n{} * 1000$; stake itself is divided equally amongst replicas (\textit{Scrooge-Large}).
(ii) Two \RSM{s} where one replica holds $50\%$ stake and the remaining $50\%$ stake is divided among all the other replicas. All replicas continue to have equal computing power. We consider this an "unfair" setup as the node with high stake does not computing power or networking bandwidth commensurate with its higher stake. It is thus a bottleneck for the system.(\textit{\Scrooge-Unfair})
(iii) Two \RSM{s} where one replica holds $50\%$ stake and the remaining $50\%$ stake is divided among all the other replicas. All replicas continue to have equal computing power. (\textit{\Scrooge-Fair}, \textit{\ATA-Fair}). We artificially bound the network throughput of all replicas with low stake to \SI{1}{Gbits\per\sec} using TC~\cite{tc}. \nc{Fix problem here?}


We make three observations. First, \ATA{}'s performance is not affected by stake when all replicas continue to have equal compute power as it requires every replica to send all messages. Second, \Scrooge-Large has identical throughput to the equal stake case. This is also expected, as \Scrooge{}'s apportionment and LCM logic will reduce the message sending/receiving pattern back to the fully equal stake case. Third, we find that unequal stake \textit{combined with equal compute} causes \Scrooge{}'s performance to drop (by $33\%$ for \Scrooge-Graded and $87\%$ for \Scrooge-Unfair) as the communication load is no longer balanced across replicas. This effect is especially pronounced in \Scrooge-Unfair where the one replica with $50\%$
has to  both send 50\% of the messages to the other RSM as well as receive messages from 50\% of the other \RSM{}'s replicas. All replicas were already networked-bottleneck in the equal stake scenarios.
In practice, nodes with higher stake typically have more computing power, as they are expected to do more work in the system. If we instead look at \Scrooge-Fair results, where the machine with the highest stake has 10x higher bandwidth than the other nodes, Scrooge outperforms \ATA-Fair by $5\times$ (small) and $8\times$ (large).
\begin{figure}[t]
    \centering
    %\resdbCCCTp
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc}
    \hspace{-8mm}\algoCCCTp  & \resdbCCCTp   & \raftCCCTp
    \end{tabular}
    \caption{Throughput \Algo{} (A), \ResDB{} (B), and \Raft{} (C)
    with Scrooge; $\n{}=4$ replicas}
    \label{fig:systems}
\end{figure}
\subsubsection{Real-World Implementations}
[TODO - GeoBFT message overhead, Kafka scaling issues. INSERT GRAPH HERE]
\nc{Don't understand what this section is for?}

\subsection{Performance under failures}
We first consider crash failures before investigating the impact of Byzantine failures.
\begin{figure}
        %\vspace{-5mm}
    \centering
    \setlength{\tabcolsep}{1pt}
    \scalebox{0.6}{\ref{mainlegend2}}
    \scalebox{0.6}{\ref{mainlegend3}}\\[5pt]
    \begin{tabular}{cc@{\quad}cc}
    \graphFStake & \graphFail
    \end{tabular}
    \caption{Analyzing effect of stake and failures on \Scrooge{}.}
    \label{fig:file-stake-fail}
\end{figure}

\par \textbf{Crash Failures} 
We conduct a simple experiment in which we randomly crash 33\% of the replicas in each RSM. We consider a message size to \SI{1}{MB} and increase the number of replicas from $4$ to $19$ (results are similar for smaller messages.)  We find that \Scrooge{} continues to outperform \ATA{} by $1.93\times$ on small networks (size 4), and up to $6.6\times$ on larger networks. 
\Scrooge{}'s performance with failure is lower than the non-failure case because a third of each message must be resent, using up both CPU and bandwidth. Interestingly, \ATA{}'s performance does not degrade during failures: \ATA{}, in effect, preemptively assumes that replicas may fail and thus always has all replicas send all messages all the time. \nc{TODO discuss this}

\par \textbf{Byzantine Failures}
Next, we consider the impact of Byzantine failures in the system. 
There are three main types of attacks. Malicious nodes can 1) send invalid, uncommitted messages 2) send incorrect quorum acknowledgements
3) collude to selectively drop messages.i
\nc{NOT YET DONE WITH REWRITE}
\begin{enumerate}[nosep,wide]
    \item \textbf{Send uncommitted messages.} Malicious replicas can send garbage messages to nodes on the receiving RSM. However, replicas in \Scrooge{} will never rebroadcast a message unless it carries a proof that the message was committed in the sending RSM. Consequently all uncommitted messages will be ignored. This attack is effectively equivalent to a DDOS attack and not something that any BFT protocol can defend against.
    \item \textbf{Sending incorrect acknowledgements.} 
    Correct nodes wait for a quorum of $u+1$ matching acks in order to consider the message delivered. They thus effectively assume that $u$ of those acks will be lies. Lying about an ack (instead of telling the truth) thus delays the formation of a quorum. Failing to send an ack delays the formation of a quack in the same way. Figure 9ii shows that, even when crashing the max number of nodes, Scrooge still has good performance.  We can add an experiment that has byzantine nodes lie about acks as well; we expect it to have the same performance.
    \item \textbf{Colluding to repeatedly drop messages.} Scrooge assumes (and ensures) that node ids are assigned to nodes using a verifiable source of randomness. The Dynamic Sharewise Scheduler (DSS: section 5.2) then computes which nodes will send what messages solely with node IDs and message sequence numbers. Collusion is thus ineffective. At worst, a DSS schedule may permit at most $u_{sender}+u_{receiver}$ retransmissions. This many retransmissions is unavoidable by any strategy as $u_s$ senders may fail and $u_r$ receivers may fail (Lemma 1 supplementary-material). However, Theorem 1 shows that Scrooge, with high probability, will never drop a message more than 72 times even if $u_{sender}+u_{receiver}$ is unbounded, minimizing Byzantine influence.
\end{enumerate}
\nc{TODO: rewrite when we have graphs. I don't think we need to talk again about Aardvark here, we have in the past already a lot}
[INSERT GRAPHS AND EXPLANATION OF EXPERIMENTS HERE, also add in "Baseline" line to graph and describe it in the text]
The design of Scrooge has been greatly influenced by the lessons of Aardvark \cite{aardvark}. True to Aardvark's spirit, Scrooge does not have an optimistic path that defers work to the failure path (like Zyzzyva \cite{zyzzyva} and other speculative approaches do). Instead, we are pessimistic and always include sufficient information ($\phi$-lists) to retransmit missing messages. Our evaluation shows we perform well even with the maximum number of failures (Figure~\ref{fig:file-stake-fail}(ii)). As Scrooge fully leverages the bandwidth of all nodes, killing a node naturally comes with a performance cost; this is fundamental. Nonetheless, in the failure case our performance still shines (6.6x vs ATA).





% message_size,latency,throughput,strategy,local_network_size,foreign_network_size
% 1000000,0,27.883312317815374,All-to-All,4,4
% 1000000,0,15.900000265000221,All-to-All,7,7
% 1000000,0,10.96667416056202,All-to-All,10,10
% 1000000,0,0.033333346666672,All-to-All,13,13
% 1000000,0,6.483335269446867,All-to-All,16,16
% 1000000,0,5.249999740000131,All-to-All,19,19
% 1000000,0,105.69999656000023,Scrooge k=64+ resends,4,4
% 1000000,0,104.69998509334587,Scrooge k=64+ resends,7,7
% 1000000,0,76.16668948779224,Scrooge k=64+ resends,10,10
% 1000000,0,89.3000304216826,Scrooge k=64+ resends,13,13
% 1000000,0,48.43330666669511,Scrooge k=64+ resends,16,16
% 1000000,0,44.01666936891273,Scrooge k=64+ resends,19,19

\subsection{Case Study: \RSM{}-to-\RSM{} in the Wild}
In this section, we illustrate several real-world use cases where \RSM{}-to-\RSM{} communication is 
necessary and \Scrooge{} can facilitate efficient communication between these \RSM{s}.

{\bf (1) Disaster Recovery.}
To recover from a disaster that causes an \RSM{} to fail, 
organizations need to copy data from the failed \RSM{} to an available \RSM{}~\cite{disaster-recovery-confluent}.
For instance Confluent needs to copy data between two \Raft{} \RSM{s} under disaster recovery.
We run a disaster recovery scenario using \Scrooge{} to communicate messages between two Etcd's \Raft{} \RSM{s} (version v3.0).
Base throughput for Raft is 39,000 tx/sec.

{\bf (2) Decentralized Finance/Blockchain.}
Cross-chain communication is quite popular in decentralized finance to support interoperability and allow users to move their assets between cryptocurrencies.
We run a blockchain interoperability experiment by deploying two \Algo{} \RSM{s}, each of which runs a pure \PoS{} consensus~\cite{algorand}.
We select \Algo{} as it has an open-source testnet for development and it is a representative \PoS{} protocol. The observed base throughput of this setup is 130 tx/second.

{\bf (3) Distributed Databases/Sharding.}
Distributed databases often increase availability and scalability by employing sharding; 
dividing data among multiple geographically-distributed shards. 
We deploy two \ResDB~\cite{resilientdb} \RSM{s} running \pbft{} consensus to simulate communication among shards. 
We select \ResDB{} as it is open-source (incubating under Apache) and provides a well-optimized \pbft{} implementation.
The observed throughput is 5000 batches/second.

{\bf (4) Distributed Trust.}
Finally, we mix-and-match different \RSM{s} and simulate a scenario where heterogeneous \RSM{s} may need 
to communicate with each other.

[TODO]
%between heterogeneous \RSM{s} (both CFT and BFT systems) to offer evidence that
%\Scrooge{} supports efficient communication between diverse, real-world \RSM{s}. 
%We consider three representative~\RSM{s}.
%\begin{enumerate}[nosep,wide]
%    \item {\bf \ResDB{}.}
%    Each \ResDB{} \RSM{} runs \pbft{} consensus to replicate  client request~\cite{geobft}.
%    We select \ResDB{} as it is open-source (incubating under Apache) and provides a well-optimized \pbft{} implementation. The observed throughput (no Scrooge) is 39,000 tx/sec.
%    \item {\bf \Algo{}.}
%    Each \Algo{} \RSM{} runs a pure \PoS{} consensus~\cite{algorand}.
%    We select \Algo{} as it has an open-source testnet for development and it is a representative \PoS{} protocol. The observed base throughput of this setup is 130 tx/second.
%    \item {\bf \Raft{}.}  Each Raft RSM runs Etcd's \Raft{} version v3.0. We select Raft as it is a popular open-source CFT consensus protocol~\cite{etcd-raft}. Base throughput for Raft is 39,000 tx/sec.
%\end{enumerate}

In Figure~\ref{fig:systems}, we present our results, which confirm that: (1) \Scrooge{} has minimal impact on the throughput of any of the \RSM{s}, with less than 15\% decrease in throughput in the worst case.
(2) \Scrooge{} successfully handles differences in throughput between RSM. The slow Algorand RSM can efficiently communicate with the much faster Raft RSM. 





%\begin{figure}[t]
%    \centering
%    \begin{tabular}{ll}
%    \hspace{-8mm}\klistTp & \hspace{-8mm}\klistLat
%    \end{tabular}
%    \caption{Performance measurements under one failure in each \File{} \RSM{s} as a function of $\phi$-list size.
%    Here, $\n{} = 4$ and message size = \SI{100}{B}.
%   }
%    \label{fig:klist-costs}
%\end{figure}



==> failure.tex <==
\section{Message Failure and Recovery}
\label{s:fail}
For yielding high throughput, \Scrooge{} prevents sending any copy 
of a message over the network. 
The Byzantine replicas can exploit this design to prevent message delivery; 
up to $\f{1}$ replicas of sending \RSM{} $\SMR{1}$ and $\f{2}$ replicas of 
receiving \RSM{} $\SMR{2}$ can crash fail or act Byzantine.
As a result, honest senders will not receiver $\f{2}+1$ cumulative \quack{s} 
for their messages.

Our \Scrooge{} protocol's zero copy policy creates an environment 
where either the sender or the receiver or both can act Byzantine and avoid detection; 
in each sender-receiver pair it is impossible to pinpoint which party is malicious.
Fortunately, malicious parties can only perform a handful of attacks on \Scrooge{}; 
a sender can only drop or indefinitely delay a message and 
a receiver can drop or avoid broadcasting message in its \RSM{}.
A consequence of these attacks is that honest receivers are unable to
extend their contiguous sets $\SAck{}$ due to missing sequence numbers. 
This stalls the communication as honest senders cannot make progress 
due to missing $\f{2}+1$ cumulative \quack{s} for some messages.
Next, we discuss how \Scrooge{} guards against these attacks.


{\bf Failure Detection.}
Once a malicious party starts dropping or ignoring messages, we need a mechanism to detect 
such an attack. 
This failure detection should be efficient otherwise it can severely degrade system performance.
%
A naive way to detect aforementioned failures is to run multiple rounds of communication 
among the replicas, where each party informs the other parties about the messages it is yet to receiver.
However, such a failure detection scheme requires exchanging $O(\n{}^2)$ messages among the replicas 
of an \RSM{} and is no less expensive than running a consensus protocol.
Further, this scheme wastes bandwidth and expects a reliable communication among the replicas. 


To this end, \Scrooge{} provides an efficient failure detection scheme, which 
requires no additional phases or number of messages between the replicas.
An honest sender replica of \RSM{} $\SMR{1}$ detects a failure when it receives 
at least $\f{2}+1$ {\em stale} cumulative acknowledgments.
Specifically, an honest sender, $l$-th replica $\Replica{1}{l}$ of $\SMR{1}$ marks 
an acknowledgment message from the $j$-th replica $\Replica{2}{j}$ in \RSM{} $\SMR{2}$ as stale if 
it previously received an acknowledgment message from $\Replica{2}{j}$.

For example, say a sender replica $\Replica{1}{l}$ receives cumulative acknowledgement ($\Ack{\Seqn}$)
for message $m$ with sequence number $\Seqn$.
When $\Replica{1}{l}$ receives $\f{2}+1$ cumulative acknowledgments from the replicas of $\SMR{2}$
for sequence number $\ge \Seqn$, 
it assumes that it has formed a cumulative \quack{} for $m$.
In the case there are no failures, $\Replica{1}{l}$ will eventually receive cumulative acknowledgments
for $m$ from all the $\n{2}$ replicas.
Let us denote the set of replicas with the help of which $\Replica{1}{l}$ reached cumulative 
acknowledgment for $m$ as $\mathcal{Q}$.

Assume cumulative acknowledgments from at least $\f{2}+1$ replicas in $\mathcal{Q}$ are $\Ack{k}$,
that is, these $\f{2}+1$ replicas have $m$ as the last message in their contiguous set.
If in response to future messages, these $\f{2}+1$ replicas again send $\Ack{k}$, 
replica $\Replica{1}{l}$ will consider this as the {\em first set of stale} acknowledgments.
This first set of stale acknowledgments informs $\Replica{1}{l}$ that the message with 
sequence number $\Seqn+1$ is missing at at least $\f{2}+1$ replicas. 
If this was not the case, these replicas would have sent $\Ack{\Seqn+1}$ or greater instead of 
sending a stale acknowledgment.

{\bf Failure Recovery.}
Once a replica $\Replica{1}{l}$ of the sending \RSM{} $\SMR{1}$ gets a set of stale acknowledgments 
for message $m$ (sequence number $\Seqn$), 
it finds the sender-receiver pair who should have sent the subsequent message $m'$ (sequence number $\Seqn+1$) 
and initiates the recovery for $m'$.
To perform these tasks, a replica of the sending cluster does not require communication with any other replica.
Instead, each replica $\Replica{1}{l}$ does the following:
\begin{itemize}[nosep,wide]
    \item It discovers the identifiers of initial sender (say $a$) and receiver (say $b$) for $m'$ using the 
    protocols described in Section~\ref{s:algo} and~\ref{s:stake}. 
    Let us denote this attempt of sending message $m'$ as $r_{m'} = 0$.
    \item For each set of stale acknowledgments, it increments $r_{m'}$, $a$ and $b$ by one 
    (may need to $\bmod$ $a$ and $b$ by $\n{1}$ and $\n{2}$, respectively).
    \item If $l = a$, then replica $\Replica{1}{l}$ sends $m'$ to replica $\Replica{2}{b}$ 
    of \RSM{} $\SMR{2}$.
\end{itemize}

As at most $\f{1}$ senders and $\f{2}$ receivers can act Byzantine, in the worse case, \Scrooge{} guarantees 
delivery of message $m'$ in at most $\f{1}+\f{2}$ sets of stale acknowledgments for $m$.








==> intro-old.tex <==
\section{Introduction}
\label{s:intro}
%Replicated services (or replicated state machines, \RSM{s}) must communicate with each other, yet cannot do so efficiently today. 
%This paper describes a practical and general-purpose method for efficiently communicating between RSMs, with constant overhead in the absence of failures, and bounded message resends under failures. 
%\nc{Upon reading it, im not sure we need this paragraph? WHat do others think?}\mk{I tend to agree. Also, the last sentence seems too specific.}

Many organizations today use replicated state machines (\RSM{}) underpinned by consensus protocols to provide reliability, fault-isolation, and disaster recovery. This includes  key-value stores~\cite{etcd-raft,tidb,cockroach}, cluster managers~\cite{kubernetes}, microservices~\cite{paxoscom, azureservicefabric,trafalgar}.
There is, however, little support for ensuring that these \RSM{s} can \textit{communicate} effectively. Yet, several applications could benefit.
Consider for example, Etcd, a popular fault-tolerant key-value store that is used to store all Kubernetes cluster data~\cite{etcd-raft}. 
Etcd to Etcd mirroring is necessary for disaster recovery; Confluent specifically highlights the use of Kafka for disaster recovery across clusters~\cite{disaster-recovery-confluent}. 
Similarly, conversations with government agencies reveal that, 
for operational sovereignty, services cannot be managed across agency borders. 
Instead, any shared information must be communicated across \RSM{s}. 
Operability is also a key consideration: the rise of blockchain technology has increased demand for
blockchain interoperability~\cite{blockchain-interoperability-survey,blockchain-interop-survey}, requiring distinct RSMs to communicate. 

%Breaking down monolithic \RSM{s} into sub-\RSM{s} can also be beneficial for performance:  GeoBFT~\cite{geobft}, for instance, 
%highlights the benefit of running sub-\RSM{s} "locally", minimizing geo-distributed communication. 

%Most organizations with an eye towards performance and organizational scaling adopt a microservice-style architecture. 
%The availability and integrity of each such service is ensured through state-machine replication: 

These examples speak of a common need: RSMs must support the ability to efficiently and reliably exchange messages with other RSMs (whether they implement the same consensus protocol internally or not). Unfortunately, there is currently no formal or practical way for two RSMs to communicate. 
Existing solutions are either ad-hoc, offer vague (and evolving) guarantees~\cite{blockchain-interop-survey}, 
rely on a trusted third-party~\cite{trustboost}), or 
require an expensive all-to-all broadcast~\cite{spanner,sharper}. The most closely related work, Aegean~\cite{aegean}, acknowledges that RSMs must communicate, but targets a different problem: nested requests in which an RSM must make an internal request to a different service while processing the first request. 

In this paper, we propose a new primitive, the \CCCFull{} (\CCC{}) that can be used by two arbitrary RSMs to communicate. \CCC{} generalizes Reliable Broadcast to guarantee that, if RSM $A$ sends $m$, at least one correct replica in RSM $B$ should receive $m$. Any implementation of the \CCC{} primitive should offer the following properties:  1) \textit{robustness under failures}:  actively malicious or crashed nodes should neither affect correctness nor cause system throughput to drop~\cite{aardvark}.
2) \textit{low-overhead in the common-case}: for efficiency, a \CCC{} protocol should send, in the failure-free case, a single message with constant metadata. 
3) \textit{generality}: arbitrary RSMs with heterogeneous sizes, communication, and fault models should be able to communicate. It should, for instance, be possible to link a Byzantine Fault Tolerant (\BFT)  protocol with a Crash Fault Tolerant (CFT) algorithm. Similarly, asynchronous and partially synchronous protocols should also be able to communicate effectively.


We then introduce \Scrooge{}, a practical \CCC{} protocol that allows for arbitrary \RSM{s} with heterogeneous communication and failure models to efficiently communicate. Designing a \CCC{} protocol that provides good performance in the failure-free case is fairly simple (leader-to-leader boradcast suffices). The challenges arise from designing an efficient protocol that \textit{remains robust to failures}~\cite{aardvark}. The key to \Scrooge{}'s good but robust performance lies in observing that the C3B problem and the goals of TCP~\cite{computer-networks-book} share similarities. TCP seeks to offer reliable, ordered delivery between two hosts in a way that dynamically reacts to congestion and anomalies in the network. To do so at low cost, TCP leverages full-duplex communication and cumulative acknowledgements (ACKs) to asynchronously detect when messages have been received. Conversely, repeated ACKs of the same message reveal message loss. \Scrooge{} takes inspiration from these techniques, and modifies them to account for the differences between C3B and TCP: 
1) unlike TCP, which is exclusively designed for point-to-point messaging, \Scrooge{} must handle many-to-many communication and 
disseminate knowledge of failed/successful message deliveries across many nodes, 
2) \Scrooge{} must ensure that no Byzantine participant will violate correctness or cause excessive re-transmissions. In contrast, TCP does not consider malicious failures: no TCP node will falsely claim to have sent or received a message.


% \Scrooge{} adopts a similar approach, but must deal with two additional challenges. First, TCP cannot handle many-to-many communication; it is exclusively designed for point-to-point messaging. Second, TCP nodes fail only by crashing. No protocol participant will falsely claim to have sent or received a message. 
% In contrast, \Scrooge{}
% must ensure that no Byzantine participant can violate correctness
% or cause excessive retransmissions.
 
 To this effect, \Scrooge{} introduces the notion of \quack{}s. A \quack{} is a cumulative quorum acknowledgement for a message $m$. It concisely summarizes that all messages up to $m$ have been reliably received by at least one correct node;
\textit{repeated} \quack{}s for $m$ indicate that the next message in the sequence was not received at the receiving RSM. For weighted RSMs~\cite{algorand},
\Scrooge{} uses \textit{apportionment}~\cite{apportionment} to fairly rotate individual sender-receiver pairs and ensures that all nodes in each RSM quickly and efficiently learn which messages have been reliably received.

Using \quack{}s in \Scrooge{} yields multiple benefits. First, it ensures \textit{generality}. It allows for \Scrooge{} to seamlessly work for crash fault tolerant systems as well as for both traditional and stake-based Byzantine fault tolerant protocols. The protocol makes no synchrony or partial synchrony assumption. Second, \Scrooge{}'s \quack{}-driven implementation has low-overhead. In the failure-free case, \Scrooge{} sends each message only once, and requires only two additional counters per-message. Finally, when failures do arise, \Scrooge{} remains \textit{robust} as its resend strategy minimizes the number of messages resent: no Byzantine node can unilaterally cause spurious message retransmissions.


%Naturally, our system has some limitations. 
%In the worst-case,  \Scrooge{} may resend messages up to $2\f{}+1$ times ($\f{}$ denotes the maximum number of nodes that can fail in an \RSM{}) 
%as the first $2\f{}$ attempts may fail since a Byzantine sender or Byzantine receiver may intentionally drop the message. 
%This is a fundamental limitation of all \CCC{} protocols. We show, however, that after only constant resends, there is already a $99.99999\%$ probability that the message has been successfully delivered. 
%Importantly, this result holds independently of network size or the value of $\f{}$. 
%The performance of \Scrooge{} under failures is thus w.h.p independent of $\f{}$.
%
Our results confirm \Scrooge{}'s strong guarantees. 
\Scrooge{} allows disparate protocols such as \pbft~\cite{pbftj}, Raft~\cite{raft} and Algorand~\cite{algorand} to communicate. In our microbenchmarks, when consensus is not the bottleneck, \Scrooge{} achieves $3.2\times$ better performance than a traditional All-to-All broadcast for small networks, and up to $24\times$ for large networks. In summary, this paper makes the following contributions:
\begin{enumerate}
    \item We introduce the \CCCFull{} primitive, which allows for two RSMs to communicate.
    \item We present \Scrooge{}, a practical \CCC{} protocol. Key to \Scrooge's good performance is the use of \quack{s} (cumulative quorum acknowledgments), which precisely determine when messages have definitely been
    received, or definitely been lost.
    \item We leverage \textit{apportionment} to ensure that the performance of \Scrooge{} is preserved in the presence of stake-based RSMs.
%    \item \mk{Just like the commented text below this says, I am still in favor of including the evaluation as an explicit contribution.}\nc{Still really hate it ;-)}
%    \item \nc{I dislike putting eval and implementation as a a contribution, but Manos would like to}\mk{The idea is that in a systems paper the performance results are part of the story and a contribution in and of themselves.}\nc{Sure, but you almost always conclude with the performance numbers - I tend to dislike it as its a contribution that says "we did our job"}
\end{enumerate}

%
%\begin{itemize}
%\item \nc{I always finds it easiest to start with a header "This paper describes the first efficient and general RSM-to-RSM communication protocol. Then you describe the context (it helps give people an idea of what you're going to talk about whe you start the background}
%There are ample scenarios where two or more organizations may 
%need to communicate with each other:
%(1) Alice may ask Robinhood to transfer all her assets to Fidelity. 
%(2) Bob may request conversion of his Ether to Algos.
%(3) Two shards need to exchange data to fulfill a cross-shard transaction.
%\item As all of these organizations need to store and exchange some data, 
%they must employ at least one Replicated State Machine (\RSM{}) to 
%reliably manage this data.
%\nc{I'd first start with why you want a  (BFT) RSM and then introduce the desire for communicate : Organisations ensure the availability and integrity of mission-critical services through replication; through \textit{state machine replication} (RSM), they offer clients the abstraction of a single correct machine in the presence of failures. More recently, increased concerns about trust and machine compromise has led companies to offer \textit{Byzantine fault-tolerant} (BFT) RSM, which are guaranteed to remain correct in the presence of arbitrary machine failures. Modern services often consist of multiple RSMS, be it for organisational or performance reasons. (Organisational) Large companies often adopt a micro-service style architecture: Uber's infrastructure consists for more than 1000 microservices. Conversations with government agencies reveal that, for security, RSMs cannot cross agency boarders, yet their systems must frequently interact. In the specific context of blockchain systems, users may want to convert Ethers to Algos. (Performance) Developers may choose to break down an RSM into multiple sub-RSMs for performance reasons: GeoBFT highlighted the benefit of running sub-RSMS "locally", minimizing geo-distributed communication. Similarly, sub-RSMs are often used as shards in a system for scalability. Supporting cross-shard transactions requires them to periodically communicate.  
%In short, BFT RSMs must support the ability to efficiently and reliability exchange messages with other RSMs.}
%\item Another common denominator in all of the aforementioned scenarios 
%is a {\em communication fabric}
%that facilitates data exchange between two organizations.
%If the communicating organizations trust each other and no failures can occur, 
%the communication problem is trivially solved.
%Unfortunately, failures are common, organizations may act maliciously, 
%and trust is often fleeting.
%\nc{It's good practice to not start a paragraph with "another point is ..", you always want to make sure that there's a directed "flow" from one paragraph to the next, suggesting that there's "another ..." means that you probably should have started the previous paragraph by "there are two issues ... " etc.}
%\nc{I'm not sure I understood the point of this paragraph?} 
%
%\item Unfortunately, existing literature lacks a concrete primitive 
%that expresses reliable communication between two organizations, and 
%includes {\em ad hoc} solutions to resolve this problem. 
%\nc{I'd say: There is currently no formal or practical way for two RSMs to communicate. Existing solutions offer vague (and evolving) guarantees~\cite{}, rely on a trusted third-party~\cite{}, or require an expensive all-to-all broadcast}
%
%\item To this end, this paper first lays down the 
%\CCCFull{} (\CCC{}) primitive. 
%Unlike reliable broadcast, which defines communication between two nodes, 
%\CCC{} expresses communication between two \RSM{s} and
%defines the necessary safety and liveness properties, 
%such as validity, no duplication, integrity and consistency.
%\nc{In this paper, we initiate the formal and practical study of the 
%\CCCFull{} problem. \CCC{} generalises Reliable Broadcast to enforce
%safety and liveness guarantees between two RSMs.}
%
%\item Next, we present our novel \Scrooge{} protocol, which correctly
%implements the \CCC{} primitive.
%\Scrooge{} is the first distributed and trustless cross-cluster 
%communication protocol, which guards against 
%malicious attacks and in the good case broadcasts {\em zero} copies of 
%each message.
%\nc{Usually, you want the system to be after the challenges, so I would move this bullet down and say "An efficient and practical \CCC{} protocol should offer the following guarantees: 1) generality
%(support arbtirary RSMs + no third-party) 2) low-overhead in the common-case (minimal additional messages sent) 3) robustness under failures}
%
%\item Prior to designing \Scrooge{}, we had to solve three key challenges
%impacting existing solutions:
%\begin{enumerate}[wide,nosep]
%\item {\em Heterogenity.}
%Two communicating \RSM{s} may differ from each other on a variety of parameters:
%(i) They could have different number of replicas, 
%(ii) They may have different failure models: crash failures vs. malicious failures.
%(iii) They could run different protocols for fault-tolerant replication. 
%(iv) They may assign different weights to different replicas to indicate priority.
%\nc{I'd move this bullet to be what you talk about in Requirement 1 above. I'd also be more precise, when you talk about weights, talk about proof of stake more directly. When you're talking about the requirements for a protocol, remember that you are talking about high level features, not Scrooge specifically: For example, we shouldn't talk about acks as there could exist a protocol implements C3PO but doesn't use acks}
%
%\item {\em Resiliency.}
%The communication fabric guaranteeing message delivery between the \RSM{s} should 
%satisfy the following properties:
%(i) It should not depend on a {\em trusted third-party}.
%(ii) It should not depend on a {\em trusted} programmable code. 
%{iii} It should continue operation despite some failures. 
%{iv} It should ensure operation under asynchrony.
%\nc{I'd move asynchrony under generality. To me, generality has two axis: composing arbitary fault-models and arbitrary communication models. Composing arbitrary communication models requires any C3PO protocol to be asynchronous. Composing arbitrary failure models requires C3PO to  ...}
%
%\item {\em Efficiency.}
%The communication fabric guaranteeing message delivery between the \RSM{s} should 
%satisfy the following:
%(i) It should be scalable.
%(ii) It should communicate {\em zero} copies of each message until failures.
%(iii) It should minimize the number of message acknowledgments. 
%(iv) It should be able to take advantage of full-duplex data flow.
%\end{enumerate}
%
%\item Unfortunately, existing solutions at most resolve one of these three challenges.
%On the one hand, solutions relying on trusted third-party or program are unsecure as 
%the trusted entity can be compromised, sink of targeted attacks, 
%or source for DOS attacks.
%Further, these solutions are extremely compute-intensive and have high latencies.
%
%\item On the other hand, existing trustless solutions create massive copies 
%of each message and expect a synchronous network.
%For example: an {\em all-to-all} protocol, 
%where all replicas in one \RSM{} send a copy of each message to all the 
%replicas in other \RSM{}, creates a total of $O(n^2)$ copies.
%Optimized variants of this protocol run expensive recovery mechanisms under failures.
%
%\nc{I agree with you that this is the right place to be a bit more detailed about existing solutions, but I would split it in "Existing solutions all fall-short. In the blockchain setting, ... In the RSM setting, all-to-all + this is the place to mention Adam as people will think of Adam and we want to make sure its clear early that it targets a different problem}
%
%\item \nc{In this work,  propose Scrooge, the first C3PO protocol that satisfies all the aforementioned requirements. You want to highlight here what are the properties that Scrooge satisfies (before going into details about Scrooge). Scrooge is asynchronous, supports RSMs of arbitrary size in the CFT, BFT model, traditional BFT + proof of stake. In the common case, sends no additional messages. In the failure case, sends at most X additional messages}
%
%Our protocol \Scrooge{} meets all the challenges.
%\Scrooge's replicas determine whether a message has been 
%delivered or not through our novel
%{\em quorum acknowledgments} (\quack{}).
%These \quack{s} assure the sender that the desired message has
%been delivered to at least one non-faulty receiver.
%As at most $\f{}$ replicas of the receiver \RSM{} can fail, a 
%\quack{} is composed of $\f{}+1$ acknowledgments.
%\nc{You are going into a lot of detail very quickly, and describing particular implementation details.  In an SOSP paper, you want to make sure to describe the key idea first. The key idea here is not quacks, that's an "example" of a technique that follows the  philosophy of the key idea. To me, (but we should discuss this), is
%that we "asynchronously" build a snapshot of what has been sent/received. We observe that what we're doing is, in effect, a reliable communication stream a la TCP, except that we are doing multiple nodes to multiple nodes communication, and that nodes can lie. The core tenants of TCP communication is to succintly summarise the state of the network + leveraging full duplex. We find that we can actually adopt much of the same techniques ...  }
%
%\item In the case of streaming applications, which require a
%continuous flow of messages, our \quack{s} can overwhelm the network. 
%As a result, our \quack{s} are {\em cumulative} in nature; 
%one acknowledgement message announces delivery of several consecutive messages.
%Moreover, unlike large messages, these acknowledgments have a small 
%constant size.
%
%\item Finally, \Scrooge{} supports full-duplex communication 
%where both the \RSM{s} can communicate messages at the same time.
%In fact, full duplex communication helps to hide the costs of 
%cumulative \quack{s} as the receiver can piggyback an acknowledgment 
%with an outgoing message.
%\nc{See comments above}
%
%
%\item \nc{I'd be great to talk about Reggie's optimisation here, with the 99.999\%, I think this is a very nice and interesting result that we should make sure we implement and put in the intro} To reiterate our claim that \Scrooge{} facilitates a high 
%performance communication among two \RSM{s}, in Figure~\ref{f:intro}, 
%we compare it against three state-of-the-art solutions: 
%(1) zk-bridge, a trusted, smart-contract bridge,
%(2) all-to-all communication protocol, and
%(3) one-to-one pairing protocol.
%The zk-bridge facilitates asset movement between two crypto-currencies
%Ethereum to Tendermint; we selected zk-bridge as it is the only 
%smart-contract bridge that has not been hacked.
%Trusteless protocols including \Scrooge{} facilitate 
%communication between two \RSM{s} running \pbft{} consensus.
%In this experiment, all the messages communicated across the \RSM{s} are \SI{1}{Mib} in size.
%For our measurements, we only take into account the latency of 
%communicating the message, and discard any costs or benefits of different
%consensus protocols.
%\nc{I'd recommending mirroring the text of past papers to introduce the evaluation section, there's usually a pretty "standard" way of doing so}
%
%
%
%
%
%\end{itemize}
%A large number of existing applications require communication between multiple clusters of replicas. 
%Examples of such applications include: 
%(i) Sharded systems where cross-shard transactions need to access data from two or more independent shards.
%(ii) Geo-replicated systems where the data is replicated across clusters, which are spread across the globe;
%these clusters need to periodically exchange data to ensure consistency.
%(iii) Two or more \Name{SMR}s running distinct consensus protocols; recent cross-chain blockchain applications
%target connecting two different blockchains and permit exchange of different crypto-tokens.
%
%Each of these applications can be viewed as a collection of independent clusters where each cluster manages its 
%own data and needs data from other clusters.
%Assume that each cluster has $\n{}$ machines.
%A naive way to exchange a message (say $m$) between two clusters is to require every machine in the sending cluster to send the
%message $m$ to every machine in the receiving cluster. 
%But, such a communication policy will result in transmitting $\n{}^2$ copies of the message $m$.
%To optimize this, a recent work shows that it is sufficient to transmit only $\n{}$ copies of the message $m$ 
%to guarantee that every machine of the receiving cluster {\em eventually} receives the message.
%Although this solution is linear in the number of machines in a cluster, 
%its use in streaming applications is still prohibitive as these applications have to continuously transmit 
%messages and this solution requires sending $\n{}$ copies per message, which will easily bottleneck the network.
%
%To resolve these challenges, in this work, we present the design of a communication protocol that 
%in the best case requires only sending {\em one} copy per message. 
%We call our protocol as {\em Shadow} as we target it for applications where clusters participate in 
%bi-directional communication (each cluster will act as a sender for some message and a receiver for another) and 
%irrespective of their nature (sender or receiver), the protocol remains the same.
%





==> motivate.tex <==
\section{Case for Cross-Cluster Communication}
\begin{itemize}[wide]
\item A large subset of present-day applications require communications 
between two or more clusters of nodes. 

\item For example, almost all the popular databases, such as Spanner, Cassandra, 
HBase, HDFS, and MongoDB implement some form of data-sharding. 
Spanner, for instance, splits data across multiple shards, where each shard runs an 
\RSM{} that employs a crash-fault tolerant (\CFT{}) consensus protocol like Paxos to 
manage state.
Cross-shard transactions force Spanner to access data from multiple shards.

\item In the financial world, it is common for users to move their assets from one 
organization to another. 
For instance, Robinhood Inc's incentives like free-stock trading and up to $\$75$ 
account-transfer remuneration has led to a large number of users switching their brokerage 
accounts to Robinhood.
Similarly, with a swelling number of cryptocurrencies, users are making use of either brokers 
like Coinbase and Binance, or smart-contract bridges to move their assets across cryptocurrencies.

\end{itemize}

\subsection{Limitations of Existing Solutions}
\begin{itemize}[wide]
\item Surprisingly, despite numerous applications requiring cross-cluster communication, 
there does not exist a primitive that explains this communication pattern. 

\item {\em Reliable Broadcast} (\Name{rb}) defines the broadcast operation by a correct sender; 
if a correct sender broadcasts a message, then eventually all correct receivers will deliver the message. 
Similarly, its variant, {\em Byzantine Reliable Broadcast} (\Name{brb}), defines 
broadcast operation under malicious failures.

\item However, these primitives do not sufficiently express cross-cluster communication 
as they mask the state of messages sent and delivered.
\Name{rb} and \Name{brb} allow an honest sender to send any message (faulty or correct) and 
only require all honest receivers to deliver the same message.

\item These primitives, when superimposed on cross-cluster communication, prevent \RSM{s} 
from guarding themselves against arbitrary messages.

\item We bridge this gap by defining \CCC{} primitive that takes into account the nature of 
messages communicated among \RSM{s}.
Specifically, an \RSM{} only sends a message $m$ if a quorum of its replicas {\em agree}
to send $m$.
To reach such an agreement, the replicas participate in a consensus protocol.


\item Although existing literature includes ad hoc implementations of \CCC{} primitive,
these implementations fail to meet all the three challenges we state in \S\ref{s:intro}.

\item For example, it is trivial for Spanner to process cross-shard transactions as it 
assumes the leader of each shard is honest and manage all communication. 
However, recent distributed systems that permit malicious leaders~\cite{aaa}, cannot rely on 
leaders for reliable cross-cluster communication.
These systems enable {all-to-all} protocol or its variants for such communications.
Unfortunately, these variants are unscalable as they create excessive copies of each message.

\item Similarly, a large subset of financial world transactions among multiple organizations 
is secured through a third-party broker or a programmable code. 
Unfortunately, relying on a third party makes this design centralized and prone to attacks; 
if the trusted entity is compromised, the resulting transactions are useless. 


\item In this paper, we present our novel \Scrooge{} protocol that meets all the challenges.
It does not trust any replica, broker, or programmable contract. 
It promotes a distributed design and guarantees zero-copy message delivery in the good case.


\end{itemize}

==> randomize.tex <==
\section{Randomized \Scrooge{}}
\label{s:random}
On the one hand, in the good case, \Scrooge{} promises message delivery without any copies. 
On the other hand, in the worst case, \Scrooge{} would require message re-transmission $\f{1}+\f{2}+1$ times.
This can lead to an unexpected observation that as failures are common, 
\Scrooge{} will always require message re-transmissions that are linear in the number of failures.
Fortunately, this is not the case, as the worst case only occurs if the adversary controls the process of assigning identifiers to the replicas.
If the adversary can ensure that $\f{1}$ Byzantine replicas of \RSM{} $\SMR{1}$ are paired with 
$\f{2}$ honest replicas of $\SMR{2}$ and 
$\f{1}$ honest replicas of \RSM{} $\SMR{1}$ are paired with $\f{2}$ Byzantine replicas of $\SMR{2}$,
then the adversary can guarantee the worst case re-transmissions for $67\%$ of messages
($\f{1}+\f{2}+1$ messages out of $max(\n{1},\n{2})$).

Prior works have shown that with the help of verifiable random functions (VRF), 
it is trivial to prevent the adversary from controlling the identifier assignment process.
Specifically, we assume that each \RSM{} employs a VRF to assign its replicas an identifier.
If this is the case, then the  Byzantine replicas will be distributed at random
and the adversary can no longer control the number of affected sender-receiver pairs.
In such setting, we show that irrespective of the value of $\n{1}, \n{2}, \f{1},$ and $\f{2}$, 
\Scrooge{} only requires a constant number of message re-transmissions under failures.

Our derivation shows that with a probability of $99.999999999\%$, for a random distribution of 
Byzantine replicas, $\Scrooge{}$ needs at most $44$ re-transmissions.
This finding is noteworthy as the value of $\f{1}$ and $\f{2}$ can be extremely larger than $44$.
Next, we show how we reach this bound.

Let,  the total number of sender-receiver pairs be $\n{1} \times \n{2}$, and
the faulty pairs be $F = \f{1} \times \n{2}  +  \f{2} \times\n{1} - \f{1} \times \f{2}$.
We know that $\f{1} < \frac{\n{1}}{3}$ and $\f{2} < \frac{\n{2}}{3}$. So, we have the following:

$F$ $=$ $\f{1} \times \n{2}  +  \f{2} \times\n{1} - \f{1} \times \f{2} < \frac{\n{1} \times \n{2}}{3} + \frac{\n{2}\times \n{1}}{3} - \frac{\n{1} \times \n{2}}{9}$

{which results in, $\frac{F}{\n{1}\times \n{2}} < \frac{5}{9}$ ~$\Rightarrow$~
$log_{\frac{5}{9}}({\frac{F}{\n{1}\times \n{2}}}) < 1$.

Now, the probability of selecting a faulty pair be $\frac{F}{\n{1} \times \n{2}}$, and
$p$ $=$ $(\frac{F}{\n{1} \times \n{2}})^q$, be the probability of selecting $q$ faulty pairs.

Combining these, $log_{\frac{5}{9}}{p}$ $=$ $q \times log_{\frac{5}{9}}{\frac{F}{\n{1}\times \n{2}}}$.

This results in $log_{\frac{5}{9}}{p} < q$.

As we want a very low probability of selecting a faulty pair, we can set $p = 1 \times 10^{-10}$ 
(this is also the probability of failures for Amazon's S3). 
This results in $q = 44$.










